Data Oblivious Algorithms for Multicores

As secure processors such as Intel SGX (with hyperthreading) become widely adopted, there is a growing appetite for private analytics on big data. Most prior works on data-oblivious algorithms adopt the classical PRAM model to capture parallelism. However, it is widely understood that PRAM does not best capture realistic multicore processors, nor does it reflect parallel programming models adopted in practice. In this paper, we initiate the study of parallel data oblivious algorithms on realistic multicores, best captured by the binary fork-join model of computation. We first show that data-oblivious sorting can be accomplished by a binary fork-join algorithm with optimal total work and optimal (cache-oblivious) cache complexity, and in O(log n log log n) span (i.e., parallel time) that matches the best-known insecure algorithm. Using our sorting algorithm as a core primitive, we show how to data-obliviously simulate general PRAM algorithms in the binary fork-join model with non-trivial efficiency. We also present results for several applications including list ranking, Euler tour, tree contraction, connected components, and minimum spanning forest. For a subset of these applications, our data-oblivious algorithms asymptotically outperform the best known insecure algorithms. For other applications, we show data oblivious algorithms whose performance bounds match the best known insecure algorithms. Complementing these asymptotically efficient results, we present a practical variant of our sorting algorithm that is self-contained and potentially implementable. It has optimal caching cost, and it is only a log log n factor off from optimal work and about a log n factor off in terms of span; moreover, it achieves small constant factors in its bounds.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=para-cache-obl-sort.pdf 
#TARGET=spaa-obl-bfork.pdf 

all: $(TARGET)

$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
#	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.log *.aux *.bbl *.blg *.out *.bak .*.xtx.cache parsetab.py \#*\# *~


==> aggreg.tex <==
\section{Aggregation, Propagation, and Routing}

Later on, our results on graph 
algorithms will need a few additional building blocks
called oblivious aggregation, propagation, and routing, respectively.
Just like oblivious sorting, these building blocks 
have been core primitives in the data-oblivious 
algorithms literature~\cite{circuitopram,opramdepth,graphsc,opram}.
%However, so far there are no known cache-agnostic implementations  
%even in the sequential setting.
%All prior known algorithms~\cite{circuitopram,opramdepth,graphsc,opram} were
%not designed for a cache-oblivious or binary-forking model.
Previously, oblivious PRAM algorithms for 
aggregation, propagation, and routing were shown~\cite{circuitopram,opramdepth,graphsc,opram};
but the earlier works did not focus on cache efficiency and their algorithms
would be a $\log n$ factor worse in 
span than ours if na\"ively converted to the binary-forking model by forking
$n$ processors per PRAM step.

In this section, we describe %how to realize these two primitives  
new cache-agnostic implementations of aggregation and propagation 
in a multi-threaded, binary-forking model.
%in the binary-forking model than our new algorithms below.


\subsection{Aggregation}

%\elaine{TODO: the definition can be strengthened: every one outputs
%the aggregated result of all elems after and including itself in the same group}

\paragraph{Aggregation for a sorted array.}
Aggregation~\cite{graphsc,opram} for a sorted array realizes the following functionality: 
given a sorted array of (key, value) pairs,
each representative element for a key
will learn some aggregation function computed over all pairs with the same key.
\begin{itemize}[leftmargin=5mm]
\item  {\it Input:}
An array ${\bf I} := \{k_i, v_i\}_{i \in [n]}$
of (key, value) pairs, %and an entry in ${\bf I}$ of the form $(\bot, \bot)$ denotes a filler element.
where some entries may be filler elements of the form $(\bot, \bot)$.
It is promised that all pairs with the same (real) key
appear in consecutive locations. 
Henceforth we refer to all elements with the same key
as the same {\it group}.
%We say that index $i \in [n]$
%is a {\it representative} for
%its group if $i$ is the leftmost element of the group.

The aggregation problem is parametrized with a publicly known,
 commutative and associative aggregation function denoted $f$ and we assume that its output range
can be stored in $O(1)$ words.
Natural examples of $f$ include summation, max, and xor.

\item
{\it Output:}
Every element learns 
its the aggregation result over all elements within its own group 
to the right of itself (itself included).
In other words, the output array ${\bf O}$
is an array also of length $n$ such that ${\bf O}[i] := f(\{v_j\}_{j \geq i, k_j = k_i} )$
if $k_i \neq \bot$; else ${\bf O}[i] := \bot$.
%contains the aggregation result for the $i$-th element.


\ignore{
The goal of oblivious aggregation is to output the following array ${\bf O}$:
\[
{\bf O}[i] := 
\begin{cases}
\left(k, f\left(\{(k, v) | (k, v) \in {\bf I} \text{ and }  k = k_i\} \right)\right) & \text{if $i$ is a representative} \\
\bot & \text{o.w.} 
\end{cases}
\]
}
\end{itemize}


\paragraph{Construction.}
We describe an oblivious algorithm for realizing aggregation. We first
describe an algorithm that is sub-optimal, but later
we can use this algorithm to bootstrap an asymptotically better one.

\begin{mdframed}
\begin{center}
${\bf Aggregate}^f({\bf I})$
\end{center}
\noindent{\bf Input:} an array ${\bf I}$ whose length $n$ is a power of $2$.
Every entry in ${\bf I}$ is of the form $(k, v)$, 
and there might be filler entries of the form $(\bot, \bot)$. It is promised
that all elements 
with the same (real) key appear in consecutive positions.
$f$ is a commucative and associative aggregation function.

%\elaine{TODO: add base case:}
\paragraph{Algorithm.}  If ${\bf I}$ has length at most $2$, perform na\"ive aggregation. 
Else, do the following:
\begin{itemize}[leftmargin=5mm,itemsep=1pt,topsep=1pt]
\item 
Divide the array ${\bf I}$ into $\sqrt{n}$ 
chunks each of size $\sqrt{n}$, denoted ${\bf I}_1, \ldots, {\bf I}_{\sqrt{n}}$.

For $i \in \sqrt{n}$ in parallel: recursively call $J_i := {\bf Aggregate}^f({\bf I}_i)$.
Each outcome array $J_i$ is of length $\sqrt{n}$.

\item 
Recursively call $K := {\bf Aggregate}^f(J_1[1] || J_2[1] || \ldots || J_{\sqrt{n}}[1])$
where $K$ is of length $\sqrt{n}$.

\item 
For each $i = 2, 3, \ldots, \sqrt{n}$ in parallel:
the tuple $K[i]$
is forwarded to each of  
$J_{i-1}[2]$, $J_{i-1}[3]$ $\ldots$, $J_{i-1}[\sqrt{n}]$. This can be performed
through forking in a binary-tree like fashion.
When the element $J_{i-1}[j] = (k, v)$ receives $K[i] = (k', v')$, it updates its own 
entry as $(k, f(v, v'))$ if $v = v'$; otherwise make a fake update.

\item 
Output the resulting $J_1, J_2, \ldots, J_{\sqrt{n}}$.
\end{itemize}
\end{mdframed}


\paragraph{Analysis.}
Correctness is not hard to verify. 
We now analyze the performance overhead of the algorithm.
As before we use $W(n)$ to denote the total work, $Q(n)$ to denote the cache complexity,
and $D(n)$ to denote the span.
\begin{align*}
\text{for } n \leq 2: \ \    &
\begin{array}{l}
W(n) = O(1) \\[5pt]
D(n) = O(1) 
\end{array}
\\
\text{for  } n \leq M: \ \  & Q(n) = O(n/B) 
\end{align*}

The recurrence is as follows:
\begin{align*}
\text{for } n > 2: \ \    &
\begin{array}{l}
W(n) = (\sqrt{n} + 1) W(\sqrt{n}) + O(n)  \\[5pt]
D(n) = 2 D(\sqrt{n})  + O(\log n)
\end{array}
\\
\text{for  } n > M: \ \  & Q(n) = (\sqrt{n} + 1) Q(\sqrt{n}) + O(\sqrt{n}) + O(n/B)
\end{align*}

Assume that $n \geq M \geq B^2$, the above  
recurrences solve to\footnote{In fact, $Q(n)$ and $W(n)$ can be bounded
a little more tightly but since we will later
bootstrap this algorithm into a tighter version anyway, we do not care about
deriving the tightest bound here.}
\[
W(n) = O(n \log n), 
\quad Q(n) = ((n/B) \log_M n), \quad 
D(n) = O(\log n \log \log n), \quad 
\]

\paragraph{Improving the asymptotical efficiency.}
Using the above ${\bf Aggregate}^f$ algorithm as a building block, we can bootstrap
an asymptotically better version. The idea
is to introduce a pre-processing and post-processing stage: 
\begin{itemize}
\item 
{\it Pre-processing}:
divide the array into chunks of size $Z = \Theta(\log n)$ (assumed
to be a power of 2), and 
perform aggregation within each chunk using 
a sequential algorithm that completes in $O(Z)$ 
sequential steps for each chunk.
%apply ${\bf Aggregate}^f$ to each chunk  first.
\item 
{\it Main step}:
At this moment, the leftmost  
element of each chunk uses its current aggregation result 
to participate 
in another aggregation problem of size $n/Z = \Theta(n/\log n)$
by calling ${\bf Aggregate}^f$.
\item 
{\it Post-processing}:
Finally, every element in the original array 
fetches the aggregation result from the next chunk's representative, 
and modifies its aggregation result accordingly.
\end{itemize}
Another way to view the above algorithm is 
basically run the earlier ${\bf Aggregate}^f$,
except that the outer-most
layer of the recursion uses a chunk size of $\Theta(\log n)$ rather than $\sqrt{n}$,
and moreover, each chunk in the outer-most layer of recursion
is solved using a simple sequential algorithm. 

The pre-processing step requires $O(n)$ total work, 
$O(n/B)$ cache complexity, and 
$O(\log n)$ span. 
The main step requires  
$O(n)$ total work, $O(n/B)$ cache complexity, and $O(\log n \log \log n)$ span.
The post-processing step requires 
$O(n)$ total work, $O(n/B)$ cache complexity assuming that $n \geq M \geq B^2$, 
%assuming that $M = \Omega(\log n)$, 
and $O(\log n)$ span.
Thus, overall, the algorithm requires
$O(n)$ total work,
$O(n/B)$ cache complexity, and $O(\log n)$ span.
We thus arrive at the following theorem:

\begin{theorem}[Oblivious aggregation]
Assume that $n \geq M \geq B^2$, and moreover $n \geq M \geq B^2$.
Aggregation can be obliviously realized
with a cache-agnostic algorithm, consuming $O(n)$ total work,
$O(n/B)$ cache complexity, and $O(\log n \log \log n)$ span.
\end{theorem}



\subsection{Propagation}

\paragraph{Propagation for a sorted array.}
Propagation~\cite{graphsc} %is the opposite of aggregation, and 
solves the following problem.
The input is an array of
${\bf I} = \{k_i, v_i\}_{i\in [n]}$
of (key, value) pairs where each (key, value) pair is either real
or filler, and a filler entry is denoted $(\bot, \bot)$.
It is promised that 
all elements with the same (real) key
appear consecutively.
We say that an element is the {\it representative} if it is the leftmost
element with its key.
%Oblivious propagation aims to achieve the following:
Now, for each key, we want to propagate
the representative's
value to all other elements with the same key.
In other words, the output 
should be an array ${\bf O}$ where 
each entry ${\bf O}[i] = (k_i, v)$ 
where $v$ is the value of the representative for the key $k_i$ in the input
${\bf I}$.
%Nayak et al.~\cite{graphsc}
%show that such oblivious propagation can be achieved in $O(\log n)$
%steps consuming $n$ CPUs where $n$ is the size of the input array.

One can realize propagation through aggregation as follows:
first, everyone entry ${\bf I}[i] = (k_i, v_i)$ 
looks to its left, and if it is the group representative,
its $w_i := v_i$; else set $w_i := -\infty$.
Now, using aggregation with the ${\tt max}$ operator, the $i$-th entry learns the 
$\max(\{w_j\}_{j \leq i, k_j = k_i})$.

We thus have the following theorem:
\begin{theorem}[Oblivious propagation]
%Assume that $M = \Omega(\log n)$, 
Assume that $n \geq M \geq B^2$.
Propagation can be obliviously realized
with a cache-agnostic algorithm, consuming $O(n)$ total work,
$O(n/B)$ cache complexity, and $O(\log n \log \log n)$ span.
\end{theorem}


\subsection{Routing}
Oblivious routing~\cite{circuitopram,opramdepth,opram,mpcformpc} solves the following problem. 
There are $n$ senders each with an item identified 
by a $(k, v)$ pair where $k$ is said to be the key, and $v$ is said to be the value. 
It is promised that the keys 
of all senders are distinct.
There are $n'$ receivers each holding a key $k$, and wants to request the item with the key $k$.
More formally, 
the input is an array $S$ of length $n$ 
where each entry 
$S[i] := (k, v)$ 
stores a data item $v$ marked with a distinct key $k$ (or a filler item with the $\bot$ key). 
Further, there is a destination array $D$ of length $n'$ 
where each entry $D[i] = k$ 
stores a key $k$, and $D[i]$ wants to request the data item 
identified by the key $k$.
%An oblivious routing algorithm routes
%the requested data item from the source array to 
%the destination array in an oblivious manner. 
The output should be an array $R$ of length $n'$, where each entry $R[i]$
stores the item with the key $D[i]$ 
if such a key exists in $S$; otherwise $R[i] = \bot$.
Note that although each destination entry is requesting a unique data item,
each source entry can send its item to many receivers.

Earlier works~\cite{circuitopram,opramdepth,opram} have shown that 
oblivious routing can be accomplished through 
$O(1)$ oblivious sortings and $O(1)$ oblivious propagation; and all the remaining
operations  
in the algorithm involve every node looking at its neighbors and performing a local
computation. Therefore, the cost is dominated by the oblivious sort. 
We thus have the following theorem:

\begin{theorem}[Oblivious routing]
Assume that $n \geq M = \log^{1+\epsilon}n \geq B^2$. %and moreover $n \geq M \geq B^2$.
Routing can be obliviously realized
with a cache-agnostic algorithm, consuming $O(n \log n)$ total work,
$O((n/B) \log_M n)$ cache complexity, and $O(\log n \log\log n)$ span.
\end{theorem}




\ignore{in our paper, we only need the simpler version
where each source routes to at most one destination, and it can be realized
with constant osort}

\ignore{
Boyle et al. [3] showed
that through a combination of oblivious sorts and oblivious aggregation, oblivious routing can be
achieved in O(n log n) total work and O(log n) parallel runtime.
In this paper, we sometimes also need a variant of the oblivious routing algorithm, a source
CPU gets informed in the end whether its block is successfully routed to one or more destination
CPUs. We elaborate how to modify Boyle et al. [3]’s oblivious 
routing building block to accomplish this.
}




==> applications-old.tex <==

\section{Applications}
We can use our new sorting algorithm to obtain efficient data-oblivious multithreaded algorithms with high cache-efficiency and
parallelism for several other problems. In Section~\ref{sec:do-app}, we discussion basic primitives for data oblivious computations.
In Section~\ref{sec:pram-app} we discuss a general PRAM emulation. Finally, in Section~\ref{sec:lr-graph}, we consider a suite
of basic graph problems, including list ranking and Euler tour, tree contraction, graph connectivity, and minimum spanning tree.

\subsection{Aggregation, Propagation, and Routing}\label{sec:do-app}

\vlr{I'll compress these definitions some more in a second pass.}
\vlr{Also, we can include these primitives in the table.}

\paragraph{Aggregation for a sorted array.}
Aggregation~\cite{graphsc,opram} for a sorted array realizes the following functionality: 
given a sorted array of (key, value) pairs,
each representative element for a key
will learn some aggregation function computed over all pairs with the same key.
\begin{itemize}[leftmargin=5mm]
\item  {\it Input:}
An array ${\bf I} := \{k_i, v_i\}_{i \in [n]}$
of (key, value) pairs,
where some entries may be filler elements of the form $(\bot, \bot)$.
It is promised that all pairs with the same (real) key
appear in consecutive locations. 
Henceforth we refer to all elements with the same key
as the same {\it group}.

The aggregation problem is parametrized with a publicly known,
 commutative and associative aggregation function denoted $f$ and we assume that its output range
can be stored in $O(1)$ words.
Natural examples of $f$ include summation, max, and xor.

\item
{\it Output:}
Every element learns 
its the aggregation result over all elements within its own group 
to the right of itself (itself included).
In other words, the output array ${\bf O}$
is an array also of length $n$ such that ${\bf O}[i] := f(\{v_j\}_{j \geq i, k_j = k_i} )$
if $k_i \neq \bot$; else ${\bf O}[i] := \bot$.

\end{itemize}

We observe that the specification for Aggregation is the same as that for Segmented Prefix Sums, a standard primitive in parallel
algorithms, which can be formulated as a prefix sums computation by augmenting each element $x$ into a pair $(x,b)$, where
bit $b$ is 1 if $x$ is the start of a group and 0 otherwise. The $f(\cdot)$ can then be suitably augmented to
another binary associative operation $f'(\cdot)$ on the element pairs
so that standard prefix sums on the pairs array  using $f'$ computes the solution to Aggregation.
The standard multithreaded prefix sums algorithm is data oblivious and runs in $O(n)$ work, $O(n/B)$ cache misses and has
$O(\log n)$ span, and these bounds apply to Aggregation. This is a considerably simpler and more efficient algorithm,
even sequentially, than earlier data oblivious algorithms for Aggregation~\cite{graphsc,opram}.


\paragraph{Propagation for a sorted array.}
Propagation~\cite{graphsc} 
solves the following problem.
The input is an array of
${\bf I} = \{k_i, v_i\}_{i\in [n]}$
of (key, value) pairs where each (key, value) pair is either real
or filler, and a filler entry is denoted $(\bot, \bot)$.
It is promised that 
all elements with the same (real) key
appear consecutively.
We say that an element is the {\it representative} if it is the leftmost
element with its key.
Now, for each key, we want to propagate
the representative's
value to all other elements with the same key.
In other words, the output 
should be an array ${\bf O}$ where 
each entry ${\bf O}[i] = (k_i, v)$ 
where $v$ is the value of the representative for the key $k_i$ in the input
${\bf I}$.

Similar to Aggregation, Propagation can be formulated as a Segmented Prefix Sums problem and hence has the same
optimal bounds: a data oblivious cache-agnostic deterministic algorithm with $O(n)$ work, $O(\log n)$ span and $O(n/B)$ cache misses.

\begin{theorem}\label{thm:aggreg-prop}
Both 
Aggregation cand Propogation for a Sorted Array can be obliviously realized
optimally with a cache-agnostic algorithm, consuming $O(n)$ total work,
$O(n/B)$ cache complexity, and $O(\log n)$ span.
\end{theorem}

\paragraph{Routing.}
Oblivious routing~\cite{circuitopram,opramdepth,opram,mpcformpc} solves the following problem. 
There are $n$ senders each with an item identified 
by a $(k, v)$ pair where $k$ is said to be the key, and $v$ is said to be the value. 
It is promised that the keys 
of all senders are distinct.
There are $n'$ receivers each holding a key $k$, and wants to request the item with the key $k$.
More formally, 
the input is an array $S$ of length $n$ 
where each entry 
$S[i] := (k, v)$ 
stores a data item $v$ marked with a distinct key $k$ (or a filler item with the $\bot$ key). 
Further, there is a destination array $D$ of length $n'$ 
where each entry $D[i] = k$ 
stores a key $k$, and $D[i]$ wants to request the data item 
identified by the key $k$.
The output should be an array $R$ of length $n'$, where each entry $R[i]$
stores the item with the key $D[i]$ 
if such a key exists in $S$; otherwise $R[i] = \bot$.
Note that although each destination entry is requesting a unique data item,
each source entry can send its item to many receivers.

This computation can be performed with a constant number of sorts and scans as follows:




\vlr{I'll fill this in, it's quite simple.}


Hence Routing can be performed with 

\begin{theorem}[Oblivious routing]
Assume that $n \geq M = \log^{1+\epsilon}n \geq B^2$. %and moreover $n \geq M \geq B^2$.
Routing can be obliviously realized
with a cache-agnostic algorithm, consuming $O(n \log n)$ total work,
$O((n/B) \log_M n)$ cache complexity, and $O(\log n \log\log n)$ span, with all but negligible probability in $n$.
\end{theorem}


\subsection{PRAM Emulation and Minimum Spanning Forest}\label{sec:pram-app}

It is well-known that each step of a $p$-processor CRCW PRAM computation can be emulated on an EREW PRAM in $O(\log p)$ time
with $p$ processors (see, e.g.,~\cite{KR90}). This simulation uses a constant number of sorts, scans, and segmented prefix sums, and
the processors cooperate to perform the reads and writes for all processors:
We use an auxiliary array $W$ of length $p$, and
for a write, the $i$-th processor writes the pair $(m_i,val_i, i)$ in the $i$-th if it needs to write value $v_i$ in location$m_i$ in this PRAM step.
This array is sorted an duplicates removed (or resolved using the Concurrent Write rule used), and then the $i$th processor performs an exclusive
write for for the pair $(m,v)$ in $W[i]$ if that pair has not been removed. Reads are similar, except that there is a segmented prefix sums
step to broadcast a value read by multiple processors. A  cache-efficient  emulation of a PRAM step is given in~\cite{CG+95}, where they
assumed that the space used by the algorithm is the same as $p$, the number of processors. Here we consider the more general case
where the algorithm uses space $s$. Then, the cost for performing the actual reads to and writes from memory in a step is $scan(s) = O(s/B)$
since the memory locations to be accessed are in sorted order. Hence the caching cost of the reads and writes is $O(sort(p) + scan(s))$, with
the cost of the rest of the emulation being bounded by $O(sort(p)$.
Thus we have the following theorem.

\begin{theorem}\label{thm:pram-emul}
Consider a single parallel CRCW PRAM step with $p$ processors, consisting of parallel reads from memory, followed by unit-time local computation,
and then parallel writes to memory. If the space used by this computation is in $s$ contiguous locations in memory, then this step
can be data-obliviously realized with a cache-agnostic algorithm with $O(p \cdot \log p)$ work, $O(sort(p) + scan(s))$ cache complexity,
and span $O(\log p \cdot \log\log p)$, with all but negligible probability in $p$.
\end{theorem}
\vlr{I think tree contraction bounds using this theorem match the bounds you obtained (since the space decreasing geometrically). 
We can still put your write-up in the appendix as
an explicit algorithm instead of a general simulation.}

We can now use the data-oblivious algorithms we have seen for the steps in this emulation algorithm, to convert
any PRAM algorithm (CRCW or EREW) that runs in $T(n)$ parallel steps with $p(n)$ processors using $s(n)$ space 
into a data-oblivious multithreaded algorithm with binary forks and joins with $O(T(n) \cdot p(n) \cdot \log n)$ work, 
$O(T(n) \cdot  (sort(P(n) + scan(s(n)))$ cache-agnostic
caching complexity, and $O(T(n) \cdot \log n\cdot \log\log n)$ span.


A concrete application of this result is in computing connected and minimum spanning forest (MSF)  in an undirected graph (edge-weighted 
graph for MSF) on $n$ nodes and $m$ edges. Both of these problems can be solved optimally in $T(n)=O(\log n)$ parallel time and $O(m+n)$ work and
space on an EREW PRAM w.h.p in $n$~\cite{PR02}.
\vlr{I need to check if this can be made all but negligible probability.}
Hence we have $p(n) = (m+n)/\log n)$ and $s(n) = O(m+n)$, leading to the following theorem
using the above emulation.

\begin{theorem}\label{thm:conn-msf}
Connected components and minimum spanning forest in a graph with $n$ nodes and $m$ edges can be computed  
with $O((m+n) \cdot \log n)$ work, $O(sort(m+n) + \log n \cdot scan(m+n))$ cache-agnostic caching cost, and
$O(\log^2 n \cdot \log \log n)$ parallel time. The data obliviousness holds with all but negligible probability in $n$,
and the performance bounds hold w.h.p. in $n$, i.e., with probability greater than $1-1/n^k$, for a constant $k$.
\end{theorem}

This result improves over the previous best results for these problems~\cite{BGS10,CR12} by
reducing the work and parallel time by a logarithmic factor and reducing the caching overhead (relative to the optimal sort bound) to 
$\log n \cdot n/B$ instead
of the earlier $\log \cdot (n/B) \log_M n)$.



In the next subsection we give data oblivious algorithms for well-studied list-ranking and Euler tour  problems with  bounds that  are better than the ones we can obtain by the PRAM emulation.
We also present a data oblivious implementation of tree contraction and connected components through explict algorithms that
match the bounds that can be obtained through~\ref{thm:pram-emul}.

\vlr{I guess we should put in a theorem for tree contraction as well.}
\vlr{Actually, the Shiloach-Vishkin algorithm will be worse by a log factor on the work.}


We now turn to list ranking and Euler tour.

\paragraph{List Ranking and Euler Tour}

\vlr{I'll fill this in later today. I don't know why the above line shows up colored.}







==> applications2-old.tex <==
%\section{List Ranking and Graph Algorithms}

\section{Applications}
\label{sec:apps}
We describe various applications of our new sorting algorithm, including
list ranking, Euler tour and tree functions, tree contraction, connected components,
and minimum spanning forest. 
%VLR: 
% Intrigingly, 
Some of our data-oblivious algorithms asymptotically outperform
the previous best known insecure algorithms (in the cache-agnostic, multithreaded setting)
\VLR{I think all of our results at least match the previous best, so I re-worded.}
%Others 
while the rest of our results
match the previous best known insecure results. 

\subsection{List Ranking}

In the list ranking problem we are given an $n$-element linked list on the elements $\{1, 2, \ldots , n\}$.
The linked list is represented by the successor array $S[1..n]$, where $S[i] = j$ implies that element 
$j$ is the successor of element $i$. If $i$ is the last element in the linked list, then $S[i]$ is
set to 0.
Given the successor array $S[1..n]$, the list ranking problem asks for the rank array $R[1..n]$,
where $R[i]$ is the number of elements ahead of element $i$ in the linked list represented by
array $S$, i.e., its distance to the end of the linked list. 
%VLR   
In the weighted version of list ranking, each element has a value, and needs to compute the sum of the values at elements ahead
of it in the linked list. Both versions can be solved with essentially the same algorithm.

To realize list ranking obliviously, 
we first apply an oblivious random permutation to randomly permute the input array. 
Then, every entry in the permuted array calculates its new index 
through an all-prefix-sum computation --- we assume that each entry also carries
around its index in the original array.
Now, every entry in the permuted array requests
the permuted index of its successor through oblivious routing. 
At this point, we can apply a non-oblivious list ranking
algorithm such as \cite{CR12}.
Finally,  
every entry in the permuted array routes the answer back to the original array
and this can be accomplished with oblivious routing.


%VLR
\hide{

%, matching the performance of the best-known, non-private algorithm: \elaine{cite}
\begin{itemize}[itemsep=1pt]
\item 
Tag each element in the input array $S$ with its index in the original array.
We may now assume that each entry of the array $S$ is of the form 
$S[i] := (i, j)$, meaning that $j \in [n]$ is the successor of element $i\in [n]$.
This can be accomplished using an all-prefix-sum computation.

\item 
Apply ORP to randomly permute the array $S$ without leaking the permutation $\pi$, and let the result be $S'$.

\item 
Each element in $S'$ now tags itself with its index 
within $S'$. This can be accomplished with an all-prefix-sum computation. 
We may now assume that each element in $S'$
is a triplet where $S'[\pi(i)] = (i, j, \pi(i))$.
%where $i \in [n]$ denotes the element, $j \in [n]$ denotes $i$'s successor, and $k$ denotes 
%its index in the permuted array $S'$.

\item 
Create the array $T$ where $T[\pi(i)] = (i, \pi(i))$ by copying $S$ by removing the middle  
field of each entry.
Now, invoke an instance of oblivious routing
where each element in $S'$ of the form $(i, j, \pi(i))$
wants to receive $\pi(j)$ from the entry $(j, \pi(j))$
in $T$. From known work~\cite{circuitopram,opramdepth}, we know 
that such oblivious routing can be accomplished by invoking oblivious sorting
$O(1)$ number of times.

The output of this step is an array denoted $U$ 
where $U[\pi(i)] = (i, j, \pi(i), \pi(j))$.

\item 
Now, invoke a non-data-oblivious list ranking algorithm~\cite{CR12,owdepthco}
on the array $U$, where the successor of $U[\pi(i)] =  (i, j, \pi(i), \pi(j))$ is $\pi(j)$ (and all other
fields of $U$ are ignored by the list ranking algorithm).
\elaine{need to argue that this is secure.}

As a result, each element in $U$ learns 
its distance from the end of the list.  We may view the outcome as an array $V$
where $V[\pi[i]] = (i, j, \pi(i), \pi(j), D)$, and the last field $D$ denotes
the distance from the end.

\item 
Finally, sort the array $V$ by the first field, and in the outcome array, remove all other fields 
besides the distance $D$.
Output the result.
\end{itemize}

In the above algorithm, the overhead is dominated 
is the non-private list ranking
step, which needs to invoke sorting $O(\log n)$ times
on arrays of 
%VLR
%exponentially 
geometrically
%
decreasing sizes.
Therefore, the total span of the algorithm is $O(\log^2 n \log \log n)$, 
the cache complexity is $O((n/B) \log_M n)$, and 
the total work is $O(n \log n)$.
}% end hide

We thus have the following theorem and we
match the state-of-the-art, non-oblivious, cache-agnostic, parallel 
list ranking algorithm~\cite{CR12}.

\begin{theorem}[List ranking]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$. 
Then, we can obliviously realize 
list ranking achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}

%VLR: Moved this above
\hide{
\subsection{Graph Algorithms}
Some earlier works also considered oblivious graph algorithms~\cite{oblgraph00,oblgraph01,blantongraph},
including 
Euler tour and tree contraction~\cite{oblgraph00,oblgraph01}.
However, these
prior works focus on a sequential setting and their algorithms are 
inherently sequential in nature.
%To the best of our knowledge, we are the first
%to explore oblivious graph algorithms {\it in any parallel setting}.
}% end hide

\subsection{Euler Tour}
In the Euler tour problem we are given an unrooted tree $T$, where each edge is duplicated, to
represent the two edges corresponding to a forward and backward traversal of the edge in depth first traversal of the tree,
when rooted at some vertex. This multigraph representation of $T$ has an Euler tour
since every vertex has even degree. 
The goal is to create an Euler tour on the edges of $T$ by creating a linked list on these edges, where the successor of each edge is
the next edge in the Euler tour. 

In the standard (non-oblivious) parallel algorithms literature,  the input is assumed to be 
represented by
circular adjacency lists $Adj(v)$ where %$v \in V(T)$. 
$v$ is a vertex in $T$. Specifically, $Adj(v)$ 
stores all the edges of the form $(v, *)$ in a circular list.
Also, for each edge $(u,v)$ in $Adj(u)$ it is assumed that there is a pointer
to its other copy $(v,u)$ in $Adj(v)$ (and vice versa).
For each edge $(u,v)$ in $T$, let $Adjsucc (u,v)$ be the successor of
edge $(u,v)$ in $Adj(u)$. 
It can be shown that if we assign the successor on the Euler tour of each edge $(x,y)$ 
as $\tau((x,y)) = Adjsucc(y, x)$, 
then the resulting circular linked list is an Euler tour of $T$.  This is a 
constant time parallel algorithm on an EREW PRAM and is an $O(\log n)$ span and linear work algorithm with binary forks and joins.


To obtain cache-efficiency, we create two sorted edge-lists, one sorted by the first endpoint on each edge and the other sorted by the
second endpoint on each edge. Then the two reverses of the same edge will appear at the same position on the two lists, and
$\tau((x,y))$ can be found for edges $(x,y)$ with a scan of the two arrays. If we now use our oblivious sort for the two sorts, we
obtain a data oblivious algorithm for Euler tour that matches our sorting bound.

\paragraph{Oblivious algorithm.}
We now describe a data-oblivious, cache-agnostic and multithreded realization.
Suppose that the input is a list of edges in the tree.
Our algorithm does the following: 
\begin{enumerate}[itemsep=1pt,topsep=1pt,leftmargin=5mm]
\item Make a reverse of each edge, e.g.,
the reverse of $(u, v)$ is $(v, u)$.
\item 
Sort all edges by the 
first vertex such that every edge $(u, v)$ except the last one, by looking at
its right neighbor, 
knows its successor in the (logical) circular adjacency list $Adj(u)$.  

Use oblivious propagation 
such that the last edge in each vertex's circular adjacency list 
learns its successor in the circular list too.
\item 
Finally, use oblivious send-receive where every edge
$(u, v)$ requests $(v, u)$'s successor in $Adj(v)$.
\end{enumerate}

The above algorithm can be accomplished in the sorting bound
since the costs are dominated by the sorting.

Note that Euler tour was also considered 
in data-oblivious algorithms~\cite{oblgraph00,oblgraph01,blantongraph}
but the earlier works are inherently sequential.
%There is also earlier work on oblivious graph algorithms~\cite{oblgraph00,oblgraph01,blantongraph},
%including 
%Euler tour and tree contraction~\cite{oblgraph00,oblgraph01}.
%However, these
% focus on a sequential setting and their algorithms are 
%inherently sequential in nature.

\paragraph{Tree computations with Euler tour.}
Euler tour is a powerful primitive.  Once an Euler tour $\tau$ of $T$ is constructed, the
tree can be rooted at any vertex, and many basic tree properties such as 
preordering numbering, postorder number, depth, and number
of descendants in the rooted tree can be computing using a list ranking algorithm  
on $\tau$ (with an incoming edge to the root removed
to make it a non-circular linked list).
We can therefore obtain oblivious realizations
of these tree computations too, by invoking our oblivious Euler tour
algorithm followed by oblivious list ranking.
The performance bounds will be dominated by the list ranking step.

%\elaine{it was not clear in the intro what ET-Tree is}

%VLR: I think we can omit the following.
\hide{
Suppose that the vertices are %from the range $[n]$. 
numbered $1, 2, \ldots, n$.
The input ${\bf I}$ is an edge list of size $m$, where each entry
in the input array is of the form $(v, w, i)$, denoting
that $w \in [n]$ is the $i$-th child of $v\in [n]$.
We want to output an array $R$ where $R[i]$ stores
vertex $i$'s preorder numbering. 
The $i$-th vertex that 
is reached during a preorder traversal is said to have preorder numbering $i$.

We can accomplish Euler tour through the following algorithm:

\begin{enumerate}
\item 
{\it Add reverse edges.}
For each edge $(v, w, i) \in {\bf I}$, write down a reverse
edge $(w, v, \bot)$ where $\bot$ denotes that it is a reverse edge going back from $w$
to its parent $v$. 
Let $J$ be the concatenation of ${\bf I}$ and 
all the reverse edges.


\item 
{\it Edge numbering.}
Invoke an instance of all-prefix sum such that all edges 
in ${\bf J}$ acquires a unique index.
Henceforth, we may assume that each 
entry in the input array ${\bf J}$ is of the form $(e, v, w, i)$.
where the additional field $e \in [m]$ denotes the unique index 
of the edge.


\item 
{\it Create successor list.}
Using 
$O(1)$ number of oblivious routings, 
every edge can find and remember its successor edge during
a preorder traversal. \elaine{may need more explanation}
At this moment, obliviously sort the edge list
such that the $i$-th entry stores the $i$-th edge's successor.


\item 
{\it Weighted list ranking.}
Invoke an instance of oblivious weighted list ranking, 
such that each edge learns its
distance from the beginning in the list (where distance is defined
as the sum of the weights so far to reach the current edge).

\item  
{\it Send preorder number to vertices.} 
Every edge that is %either of type ${\tt LeftChild}$ or ${\tt RightChild}$
a forward edge gives its number to the vertex the edge travels to.
This can be done through 2 oblivious routings.
The first oblivious routing allows each of $n$ vertices to learn
the index of the edge coming into itself from its parent.
The second oblivious routing allows 
every vertex to receive its preorder number from this edge.
%(recall that earlier, every vertex 
%already obtained all information from its neighbors, so every vertex
%knows the index of the edge coming into itself).
\end{enumerate}


The above algorithm essentially invokes oblivious weighted list ranking
once and invokes oblivious routing, oblivious sorting, and prefix sum $O(1)$ number of times.
The performance overhead is therefore dominated by the list ranking step. 
We thus have the following theorem.

\begin{theorem}[Euler tour]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$. 
%Assume that $n \geq M \geq \log^{1+\epsilon} n$. 
Then, we can obliviously realize 
Euler tour on unbounded-degree trees achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}
}% end hide for Euler tour

%\subsection{Tree Contraction}

\vlr{I'm hiding your algorithms for tree contraction and CC, but they should be in an appendix.}
\elaine{i've  deleted my version. i don't think we need 
two different versions of the algorithm, it's too confusing.}


\hide{
\paragraph{Tree contraction.}
Tree contraction is the following problem:
given a parathesized arithmetic expression expressed as a binary-tree, 
where each leaf stores a number and each internal vertex represents
an operator, evaluate the outcome of the expression. 
We assume that the vertices in the tree are numbered $1, 2, \ldots, n$.
More specifically, the input 
is an array ${\bf I}$ where each entry ${\bf I}[i] = (l, r, {\sf expr})$
where $l \in [n]$ denotes 
the index of the left child of vertex $i\in [n]$, 
$r$ denotes the index of the right child of vertex $i \in [n]$, and 
${\sf expr}$ stores either a number 
or an expression of the form %$a l + b r + c l r + d$
$f(l, r)$ that represents
how to take the two evaluation outcomes at the children $l$ and $r$, and 
evaluate an outcome at the current vertex.
If $l = \bot$ or $r = \bot$, it means that the corresponding child does not exist for
the current vertex.

We can obtain an oblivious tree contraction algorithm 
by modifying the non-oblivious algorithm of \elaine{cite Vijaya's lecture notes} ---
to make it oblivious, the key idea is to 1) rely on oblivious routing
in each iteration for 
parent vertices to receive information from their children in parallel;
and 2) rely on oblivious sorting to remove 
defunct leaves at the end of each iteration.
We describe the detailed algorithm below.
%neighboring vertices
%to fetch information from each other in parallel. 



\begin{mdframed}
Let ${\sf Tree} := {\bf I}$.
Invoke oblivious Euler tour on ${\sf Tree}$, %and the outcome
at the end, each vertex in ${\sf Tree}$ receives its preorder numbering. 
Obliviously sort ${\sf Tree}$ by the vertices' preorder numbering.
At this moment, each entry in ${\sf Tree}$
is of the form ${\sf Tree}[i] = (j, l, r, {\sf expr})$
where $j$ is the $i$-th vertex visited during a preorder traversal,
$l$ and $r$ denote 
$j$'s left and right children respectively, and ${\sf expr}$ denotes an expression.
%is an array ${\sf r}$
%where ${\sf r}[i]$ denotes the preorder numbering of the $i$-th vertex. 
%Using a constant number of oblivious routings,  
%every vertex writes down its immediate parent $p$, and it's grandparent $g$.
%We may now assume that every entry in ${\sf Tree}$ is of the form 
%$(l, r, p, g, {\sf expr})$.
%If $l$, $r$, $p$ or $g$ is $\bot$, it means that the 
%corresponding vertex does not exist.


For $i = 1, 2, \ldots, \ceil{\log_{3/2} n}$:
\begin{itemize}[topsep=1pt,itemsep=1pt]
\item 
Using $O(1)$ number of oblivious routings, every vertex in ${\sf Tree}$ 
receives the information held by both children.

\item 
All vertices in parallel do the following:
if the left child is a leaf and has an odd preorder number, then 
the vertex replaces itself with a shunted vertex (and information of the shunted
vertex can be computed from the two children's information).
\elaine{TODO: explain shunt}

\item 
All vertices in parallel do the following:
if the right child is a leaf and has an odd preorder number, then 
the vertex replaces itself with a shunted vertex (and information of the shunted
vertex can be computed from the two children's information).

\item 
Every vertex in ${\sf Tree}$  
that is a leaf with an odd preorder number 
marks itself as a filler, i.e., effectively deleted. 
Every vertex in ${\sf Tree}$  
that is a leaf with an even preorder number 
divides its preorder number by $2$.

\item 
Obliviously sort ${\sf Tree}$ to remove 
all filler entries to the end, truncate ${\sf Tree}$ preserving 
only the first $\ceil{|{\sf Tree}|/2}$ elements.
%\elaine{truncate array length}
\end{itemize}

Finally, output the expression at ${\sf Tree}[1]$.
\end{mdframed}


The above algorithm begins by invoking oblivious 
Euler tour once and oblivious sorting once; 
afterwards, each of the $O(\log n)$ iterations
invoke oblivious routing and oblivious sort 
$O(1)$ number of times on arrays of exponentially decreasing sizes. 
Thus, it can be implemented in 
$O(\log^2 n \log \log n)$ span, 
$O((n/B) \cdot \log_M n)$ cache complexity, and
$O(n \log n)$ total work.


\begin{theorem}[Tree contraction]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$.
Then, we can obliviously realize 
tree contraction achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
\end{theorem}


\paragraph{Connected components.}
Connected components is the following problem: 
suppose that the vertices are indexed by $[n]$.
The input is an array ${\bf I}$ where each entry 
${\bf I} = (u, v)$ denotes an edge in the graph.
The output is an array ${\bf O}$ where ${\bf O}[i]$
denotes the connected component vertex $i \in [n]$
belong to. It should be the case that all vertices belonging to
the same connected component 
receive the same number in the output array.

We describe a cache-agnostic, oblivious algorithm for accomplishing 
connected components. 
Our algorithm follows the blue-print of Shiloach 
and Vishkin~\cite{vishkinCC}, but we realize the communication steps
between vertices and edges.
At a very high level, in their algorithm, a core data structure 
is a parent-pointer graph: every vertex $v$ stores 
their current parent henceforth denoted $p(v)$, and updates its pointer throughout the algorithm.
At the end of the algorithm, the parent-pointer
graph is guaranteed to produce one star per connected component
where every vertex in the same connected component points to 
a ``root'' of the connected component, where the root is the representative
of the connected component. 
The root's index will become 
the connected component's identifier
assigned to the vertices belonging to this connected component.

Initially, all vertices point to themselves.
Now, 
Shiloach and Vishkin's algorithm~\cite{vishkinCC}
proceeds in $O(\log n)$ iterations, and during each iteration,
the following actions take place:
\begin{itemize} 
\item 
{\it Shortcutting}: every vertex %might decide to connect to its 2-hop parent.
in parallel updates its parent pointer to its grandparent, i.e., $p(v) \leftarrow p(p(v))$, 
if the grandparent is different
from the parent. Moreover, the new parent gets notified that some new vertex
has pointed to it. 

\item  {\it Conditional hooking.}
%If a vertex $v$'s did not update its parent the earlier step, and 
%the parent $p(v)$ has a greater index than 
%$v$'s neighbor's parent, 
If a vertex $v$'s parent $p(v)$ did not receive any new children in the previous step
(i.e., $v$ is in a star at the beginning of this iteration), 
then update 
$p(v)$'s pointer to point to 
a neighbor's parent which is smaller, i.e., 
if $(u, v)$ is an edge in the graph, $p(u) < p(v)$, and moreover $p(v)$ was not
updated in the earlier step, then update
$p(p(v)) \leftarrow p(u)$ --- if multiple such updates are made
to $p(v)$, an arbitrary one of them will succeed; moreover,
this vertex who got hooked onto will  get notified that some vertex
has newly pointed to it.

\item  {\it Unconditional hooking.}
%The root of a tree (i.e., the vertex's parent is itself) 
%is said to be stagnant if it did not get any new children, or hook onto a new parent so far
%during this iteration.
If a vertex $v$'s parent $p(v)$ did not receive any new children so far in this  
iteration (i.e., the vertex is in a star at the beginning of the iteration), 
%If a vertex $v$'s parent is a stagnant root, 
and moreover, the vertex
$v$ has a neighbor $u$ in the graph such that $p(u) \neq p(v)$, then 
update $p(p(v)) \leftarrow p(u)$. If multiple such neighbors exist, choose an arbitrary one's
parent to hook onto.
%the corresponding tree 
%is called a stagnant tree.

%\item 
%{\it Second shortcutting.}
%Repeat the shortcutting step mentioned above.
\end{itemize} 

To implement their algorithm obliviously, it suffices to show how to 
accomplish the following communication primitives obliviously:
\begin{enumerate}[itemsep=1pt,topsep=1pt]
\item 
For each vertex to in parallel receive information from its parent. %(or grandparent resp.).
This is needed for the vertex to %decide whether to shortcut to the grandparent.
find out who its grandparent is during the shortcutting steps. 
%, and decide whether to shortcut to the grandparent. 

\item 
For each vertex to 
in parallel  aggregate information from all of its 
neighbors in the original graph, or from its children in the parent-pointer graph. 
This is needed for each vertex to find out if there is a neighboring tree
for its parent to hook onto, and is needed for the root 
to learn which other tree to hook onto.
This is also needed for a vertex to learn %if it is stagnant.
if any new vertex has newly pointed 
to itself.
\end{enumerate}

To realize the above steps, our algorithm is partly 
inspired by Nayak et al.~\cite{graphsc} who
studied oblivious algorithms in an EREW PRAM model.
Imagine that our algorithm maintains a joint edge/vertex list denoted $L$
containing two types of entries.
Each vertex entry stores 
a vertex's index, its parent pointer, and 
additional information gained during in the algorithm 
(e.g., the parent of some neighbor, the iteration in which the vertex's parent
was last updated, and the iteration in which the vertex last received new children).
Each 
edge entry stores an edge in the original graph.
Moreover, the undirected edge
$(u, v)$ appears twice, once as $(u, v)$ and 
the other times as $(v, u)$. 
\ignore{
\begin{itemize}
\item 
{\it Vertex entry:}
there are $n$ vertex entries, each of the form $({\tt vertex}, i, p, {\sf payload})$
where ${\tt vertex}$ denotes the type of the entry,
$i \in [n]$ 
denotes the vertex's index, $p$ denotes its parent, and ${\sf payload}$
stores 
additional information gained during in the algorithm (e.g., the parent of some neighbor $u$).  

\item 
{\it Edges in the original graph:}
The list also contains all the $m$ edges in the original graph,
where each undirected edge 
$(u, v)$ appears twice, once as $({\tt edge}, u, v)$ and 
the other times as $({\tt edge}, v, u)$. %\elaine{is this needed}
\end{itemize}
}
Observe that the length of the list $L$ is $n + 2m$
where $n$ denotes the number of vertices and $m$ denotes the number of edges
in the original graph.
\elaine{say somewhere that we leak only n and m for all the graph algorithms}


Now, type-1 communication where each vertex receives information from the parent can be 
realized
through oblivious routing, where every vertex-entry 
in $L$ wants to fetch the entry identified by the parent's index.
Type-2 communication 
can be implemented through a combination of oblivious sorting and oblivious aggregation.
Suppose that each vertex wants to aggregate information from each neighbor
in the original graph.
This can be accomplished as follows: 
obliviously sort the array $L$ such that for each vertex $v \in [n]$,
the unique vertex
entry for $v$ appears first, followed by all edges $(v, *)$.
Now, run 
an oblivious aggregation algorithm for each 
vertex to  
aggregate information from all of its neighbors.

For a parent to aggregate information from all of its children
is similar but slightly more complicated:
notice that every vertex entry also stores an edge in the 
parent-pointer graph.
To perform the aggregation, each vertex entry must first  
replicate itself into two entries, one serves
as a vertex and the other serves as an edge --- moreover, this must
be done in a way that preserves obliviousness: 
\begin{itemize}
\item 
First, rely on oblivious sorting so all $n$ vertex
entries appear in the front of $L$.
Now, the first $n$ entries in $L$ replicates a temporary copy of itself which
represents an edge in the parent-pointer graph.
At this moment, the array $L$ is temporarily expanded to a length of $2 n + 2m$.

\item 
Obliviously sort the expanded list $L$ 
such that every vertex $v$ appears immediately in front of
all edges going into $v$ in the parent-pointer graph.
\item 
Use oblivious aggregation for all vertices to aggregate information from their children
in the parent-pointer graph.
\item 
Finally, use oblivious sorting to move all temporary copies
of vertex entries created above to the end of the array,  
and truncate those entries away. The resulting array would again be $n + 2m$ in size.
\end{itemize}


Using the above algorithms to implement the parallel communication
steps in Shiloach and Vishkin~\cite{vishkinCC},
we obtain a cach-agnostic, oblivious algorithm for connected components
as stated in the following theorem:

\begin{theorem}[Connected component]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$, and let $m$
denote the number of edges in the graph.
Then, we can obliviously realize 
connected component achieving span $O(\log^2 m \log \log m)$,
cache complexity $O((m/B) \log_M m \log m)$, and
total work $O(m \log^2 m)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}


\paragraph{Minimum spanning forest.}
The input is an edge array ${\bf I}$ where each entry ${\bf I}[i] = (u, v, w)$
stores an edge of the graph $(u, v)$ and it weight $w \geq 0$.
We may assume that all vertices have indices from the range $[n]$.
The output is a bit array ${\bf O}$
where ${\bf O}[i] = 1$ 
means that the $i$-th edge in the input array is in the minimum-weight spanning forest.

Minimum spanning forest can be computed using a very similar algorithm 
as the aforementioned connected components algorithm. 
%The only difference is that during each of the $O(\log n)$ iterations, nodes 
Initially, everyone's parent pointer points to itself.
Next, repeat the following for $O(\log n)$ iterations:
\begin{itemize}
\item {\it Shortcutting.}
Same as before.
\item  {\it Conditional hooking.}
%If a vertex $v$'s did not update its parent the earlier step, %and $v$ is in a star, 
For a vertex $v$, if 
$p(v)$ did not receive 
any new children in the previous step (i.e., the vertex was in a star
at the beginning of this iteration), 
then let $S$ be the set of $v$'s neighbors in the original graph 
such that for $u \in S$,
$p(u) \neq p(v)$.
Find the $u^* \in S$ 
whose edge weight is the minimum, 
and send $((v, u^*), w^*, p(u^*))$
to its parent $p(v)$ where $w^*$ is the weight of the edge $(v, u^*)$.

Every vertex $z$ that is a root (i.e., its parent pointer is itself)
looks at all the tuple it has received, 
choose the one with the minimum edge weight, say $((v', u'), w', p(u'))$, 
if $p(u') < p(z)$,  
 set $p(z) := p(u')$, and record that the edge $(v', u')$ is in the  minimum spanning forest.

\item  {\it Unconditional hooking.}
%The definition of a stagnant root is the same as before.
If a vertex $v$'s parent $p(v)$ %is a stagnant root, 
did not receive any new children so far in this iteration, 
let $S$ be the set of $v$'s neighbors in the original graph 
such that for $u \in S$,
$p(u) \neq p(v)$. 
Find the $u^* \in S$ whose edge weight is the minimum, 
and send $((v, u^*), w^*, p(u^*))$ to $p(v)$ if $S$ is not empty.
%and send $((v, u^*), w^*, p(u^*))$
%to its parent $p(v)$ where $w^*$ is the weight of the edge $(v, u^*)$.

Every vertex $z$ that is a stagnant root 
looks at all the tuple it has received, 
choose the one with the minimum edge weight, say $((v', u'), w', p(u'))$, 
set $p(z) := p(u')$, and record that the edge $(v', u')$ is in the  minimum spanning forest.

%\item {\it Second shortcutting.}
%Same as before.
\end{itemize}



To implement this algorithm, we can use the same techniques
as in connected components 
to implement the communication 
among neighbors (either in the original graph or in the parent-pointer graph) in each 
iteration.
The only 
additional communication is necessary is to record any edge 
chosen. This
can be accomplished through oblivious routing.

\begin{theorem}[Minimum spanning forest]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$, and let $m$
denote the number of edges in the graph.
Then, we can obliviously realize 
minimum spanning forest achieving span $O(\log^2 m \log \log m)$,
cache complexity $O((m/B) \log_M m \log m)$, and
total work $O(m \log^2 m)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}

}% end hide

\subsection{Tree Contraction, Connected Components, and Minimum Spanning Forest}
We present new results on tree contraction, connected components,
and minimum spanning forest. Intrigingly, 
our data-oblivious algorithms asymptotically outperform
the previous best known insecure algorithms (in the cache-agnostic, multithreaded setting).
\elaine{todo: cite previous papers.}

%The definitions of these problems are well-known and are deferred to the appendix where explicit data oblivious algorithms are given for them.
%We now apply the above theorem to the known PRAM algorithms for these problems to  obtain the bounds that are the same as those
%shown with explicit algorithms
%in the appendix.

%\paragraph{Tree Contraction.} 
\ignore{Vijaya, i am not very comfortable with this, i emailed you 
with the questions.
1) in Kosaraju and Delcher, is it true that the memory usage decreases at a fixed rate independent of the input? if not, it'll be tricky
2) in Kosaraju and Delcher, is there a way to look at the memory cell, and immediately know that it will no longer be needed later in O(1) CPU steps?
}

\paragraph{Tree contraction.}
The EREW PRAM tree contraction algorithm of Kosaraju and Delcher~\cite{KD97} 
runs in $O(\log n)$ parallel
with $O(n/\log n)$ processors. 
Further, the computation uses $O(n)$ space initially, 
but the number of processors as well as space needed 
decreases geometrically during $\log n$ phases,
and the rate of decrease is fixed and data independent.
Not only so, at the end of each phase, 
every memory location knows whether it is still needed in future computation;
and a constant fraction of the memory locations  
will be no longer needed at the end of each phase.

\elaine{Vijaya, can you see if this is a precise description of what you mean?}
To obtain a cache-agonostic, multi-threaded 
oblivious simulation of tree contraction, 
we can apply our earlier Theorem~\ref{thm:pram-emul}  
of Section~\ref{sec:pram-app}
in a slightly non-blackbox fashion. Basically, we use 
the strategy of 
Section~\ref{sec:pram-app} to simulate each PRAM step, 
always using the actual number of processors
needed in that step.
Additionally, we introduce the following modification:
at the end of each phase of Kosaraju and Delcher~\cite{KD97} (where each phase has 
a fixed number of PRAM steps), 
use oblivious sort move the memory entries no longer needed to the end, 
effectively removing them from the future computation.
In this way, we get the first result in  
in Theorem~\ref{thm:conn-msf} below.

Note that tree contraction was also considered
in data-oblivious algorithms~\cite{oblgraph00,oblgraph01,blantongraph} 
but the earlier works are inherently sequential. 
%There is also earlier work on oblivious graph algorithms~\cite{oblgraph00,oblgraph01,blantongraph},
%including 
%Euler tour and tree contraction~\cite{oblgraph00,oblgraph01}.
%However, these
% focus on a sequential setting and their algorithms are 
%inherently sequential in nature.

%\subsection{Connected Components and Minimum Spanning Forest}

%\paragraph{Connected Components and Graph Minimum Spanning tree.} 

\paragraph{Connected components and minimum spanning forest.}
Another important application of Theorem~\ref{thm:pram-emul} is in computing connected and minimum spanning forest (MSF)  in an undirected graph (edge-weighted 
graph for MSF) on $n$ nodes and $m$ edges. Both of these problems can be solved in $T(n)=O(\log n)$ parallel time and with $O(m+n)$ space and number of processors~\cite{Shiloah-Vishkin,PR02}.
Hence we have $T(n)= O(\log n)$,  $p(n) + s(n) = O(m+n)$, leading to the second result in the following theorem
using the above emulation. 
%This result improves over the currently best result known even for the case when data obliviousness is not needed.

\begin{theorem}\label{thm:conn-msf}
%By emulating PRAM algorithms:
Suppose that $M > \log^{1+\epsilon } (m+n)$ and $m+n \geq M \geq B^2$.
Then, we have that 

(i) Tree contraction on an $n$-node rooted tree can be obliviously realized
with a cache-agnostic, multithreaded program  
consuming 
$O(W_{\rm sort}(n))$ work, $O(Q_{\rm sort}(n))$ cache complexity,
and $O(\log n \cdot D_{\rm sort}(n))$ span. %with all but negligible probability.

(ii)
Connected components and minimum spanning forest in a graph with $n$ nodes 
and $m$ edges can be obliviously realized
with a cache-agnostic, multithreaded program
consuming
with $O(\log n \cdot W_{\rm sort}(m+n))$ work, 
$O(\log n \cdot Q_{\rm sort}(m+n))$ cache complexity, and
$O(\log n \cdot  D_{\rm sort}(m+n))$ span. % with all but negligible probability. 
\end{theorem}

\elaine{Vijaya, the definition of oblivious already 
encompasses the negligible, so you don't have to repeat the negligible any more when you
use it together "oblivious"}



\hide{
This result improves over the previous best results for these problems~\cite{BGS10,CR12} by
reducing the work and parallel time by a logarithmic factor and reducing the caching overhead (relative to the optimal sort bound) to 
$\log n \cdot n/B$ instead
of the earlier $\log \cdot (n/B) \log_M n)$.
}% end hide







==> apps.tex <==
\section{List Ranking and Graph Algorithms}

%\elaine{TODO: define oblivious routing. each receiver receives at most O(1) thing}

\subsection{List Ranking}

In the list ranking problem we are given an $n$-element linked list on the elements $\{1, 2, \ldots , n\}$.
The linked list is represented by the successor array $S[1..n]$, where $S[i] = j$ implies that element 
$j$ is the successor of element $i$. If $i$ is the last element in the linked list, then $S[i]$ is
set to 0.
Given the successor array $S[1..n]$, the list ranking problem asks for the rank array $R[1..n]$,
where $R[i]$ is the number of elements ahead of element $i$ in the linked list represented by
array $S$, i.e., its distance to the end of the linked list.

With ORP and oblivious sorting as building blocks, we can realize 
list ranking obliviously 
by first applying an ORP to randomly permute the input array and then applying a non-oblivious
list ranking algorithm on the permuted array. 
The slightly subtle detail is that after being permuted, every entry in the permuted
array needs to learn its successor's {\it permuted} index --- but this can be accomplished through
a constant number of oblivious sorts.
We describe our algorithm below:
%, matching the performance of the best-known, non-private algorithm: \elaine{cite}
\begin{itemize}[itemsep=1pt]
\item 
Tag each element in the input array $S$ with its index in the original array.
We may now assume that each entry of the array $S$ is of the form 
$S[i] := (i, j)$, meaning that $j \in [n]$ is the successor of element $i\in [n]$.
This can be accomplished using an all-prefix-sum computation.

\item 
Apply ORP to randomly permute the array $S$ without leaking the permutation $\pi$, and let the result be $S'$.

\item 
Each element in $S'$ now tags itself with its index 
within $S'$. This can be accomplished with an all-prefix-sum computation. 
We may now assume that each element in $S'$
is a triplet where $S'[\pi(i)] = (i, j, \pi(i))$.
%where $i \in [n]$ denotes the element, $j \in [n]$ denotes $i$'s successor, and $k$ denotes 
%its index in the permuted array $S'$.

\item 
Create the array $T$ where $T[\pi(i)] = (i, \pi(i))$ by copying $S$ by removing the middle  
field of each entry.
Now, invoke an instance of oblivious routing~\cite{circuitopram,opramdepth},  %\elaine{todo: fix cite}
where each element in $S'$ of the form $(i, j, \pi(i))$
wants to receive $\pi(j)$ from the entry $(j, \pi(j))$
in $T$. From known work~\cite{circuitopram,opramdepth}, we know 
that such oblivious routing can be accomplished by invoking oblivious sorting
$O(1)$ number of times.

The output of this step is an array denoted $U$ 
where $U[\pi(i)] = (i, j, \pi(i), \pi(j))$.

\item 
Now, invoke a non-data-oblivious list ranking algorithm 
such as the one described by Blelloch et al.~\cite{lowdepthco}, 
\elaine{write its performance in preliminary}
%\elaine{fix cite}
on the array $U$, where the successor of $U[\pi(i)] =  (i, j, \pi(i), \pi(j))$ is $\pi(j)$ (and all other
fields of $U$ are ignored by the list ranking algorithm).
%Recall that the list ranking algorithm by Blelloch et al.~\cite{}
%needs a sorting algorithm as a building block, and here we can instantiate the sorting 
%with any comparison-based sorting 
%algorithm that need not be data-oblivious.
\elaine{need to argue that this is secure.}

As a result, each element in $U$ learns 
its distance from the end of the list.  We may view the outcome as an array $V$
where $V[\pi[i]] = (i, j, \pi(i), \pi(j), D)$, and the last field $D$ denotes
the distance from the end.

\item 
Finally, sort the array $V$ by the first field, and in the outcome array, remove all other fields 
besides the distance $D$.
Output the result.
\end{itemize}

%In the above algorithm, we can invoke the insecure list ranking algorithm by
%Blelloch et al.~\cite{} \elaine{fix cite} --- their algorithm invokes sorting
%but we can use any non-data-oblivious, comparison-based sorting 

%It is not hard to see that the above algorithm can be accomplished 
%in $O()$
In the above algorithm, the overhead is dominated 
is the non-private list ranking
step, which needs to invoke sorting $O(\log n)$ times
on arrays of exponentially decreasing sizes.
Therefore, the total span of the algorithm is $O(\log^2 n \log \log n)$, 
the cache complexity is $O((n/B) \log_M n)$, and 
the total work is $O(n \log n)$.


We thus have the following theorem --- our asymptotical performances
match the state-of-the-art, non-oblivious, cache-agnostic, parallel 
list ranking algorithm~\cite{lowdepthco,CR17,vijayasort}.

\begin{theorem}[List ranking]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$. 
Then, we can obliviously realize 
list ranking achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}

\paragraph{Extension: weighted list ranking.}
We can extend 
the above to weighted list ranking. In weighted list ranking, 
the input $S[i] = (j, w)$
where $j$ is $i$'s successor and $w$ is the weight of the edge. 
We want to output an array $R$, such that the $R[i]$ is the total
distance (i.e., sum of the weights) if we travel 
from $i$ to the end of the list.
The same non-oblivious list ranking algorithm~\cite{lowdepthco} 
(invoked by our earlier oblivious list ranking algorithm) 
can also compute weighted list ranking.
Moreover, the algorithm's access patterns are dependent only on the structure 
of the list  but not on the weights.
Therefore, the same algorithm earlier can also give weighted list ranking
with the same asymptotical costs.


\subsection{Graph Algorithms}
Some earlier works also considered oblivious graph algorithms~\cite{oblgraph00,oblgraph01,blantongraph},
including 
Euler tour and tree contraction~\cite{oblgraph00,oblgraph01}.
However, these
prior works focus on a sequential setting and their algorithms are %not readily parallelizable.  
inherently sequential in nature.
%To the best of our knowledge, we are the first
%to explore oblivious graph algorithms {\it in any parallel setting}.


\ignore{
\paragraph{Euler tour on binary trees.} 
Given an unrooted binary-tree stored in pointer format, for each vertex, 
output its preorder 
numbering. The $i$-th vertex that 
is reached during a preorder traversal is said to have preorder numbering $i$.
More specifically, suppose that the vertices are numbered $1, 2, \ldots, n$, 
the input is an array $S[0..n-1]$
where $S[i] = (l, r)$ means that vertex $i$'s left child is 
$l \in [n] \cup \{\bot\}$ 
and its right child is $r \in [n] \cup \{\bot\}$. 
If either $l$ or $r$ is set to $\bot$, it means that 
that vertex $i$ does not have a left or right child respectively. 

We can construct an oblivious Euler tour algorithm as follows:

\begin{enumerate}
\ignore{
\item 
{\it Everyone finds its parent.}
Using oblivious routing~\cite{circuitopram,opramdepth}, every vertex 
in the list $S$ 
can find its parent. At this moment, we may assume that 
each entry of $S$ is of the form $S[i] = (l, r, p)$
which stores vertex $i$'s left child, right child, and parent respectively. A $\bot$ value means
the left child, right child, or parent does not exist.
Oblivious routing 
can be realized with $O(1)$ number of oblivious sorts~\cite{circuitopram,opramdepth}.
}

\item
{\it Edge numbering.}
Every vertex $i \in [n]$ looks at $S[i]$ writes down 
 a number that is its number of children plus 1. 
This is the total number of edges outgoing from vertex $i$, including the edges
to the children and the edge
going back to the vertex's parent. We assume that the root 
has a fake outgoing edge going to a fake parent and this fake edge acquires 
an index too.
%has a fake parent and
%an edge going back to its fake parent. 
Using all-prefix-sum, 
every vertex can assign its outgoing edges a distinct number from $1, 2, \ldots, 2n-1$.

\item 
{\it Create edge succesor list.}
Using $O(1)$ number of oblivious routings, every vertex 
can obtain all information stored by its 
1) left child, 2) right child, and 3) parent.
In this way, every vertex can write down  
$3$ entries, where each entry is 
of the form $(e, s, \tau)$
where $e$ is one of the outgoing edges of this vertex,
$s$ is $e$'s successor in the preorder traversal, and $\tau \in \{{\tt LeftChild}, {\tt RightChild}, {\tt Parent}\}$ is the edge type.
%\item 
%or $\bot$ in the corresponding positions if the vertex does not have $3$ outgoing edges.
%\end{itemize}
If the vertext does not have $3$ outgoing edges,
it still writes $3$ entries but $\bot$ is written for the outgoing edges 
that do not exist.
For the root, it will not find a parent, so for its fake parent edge, say, numbered $e$, 
the entry $(e, 0, {\tt Parent})$ is written.



At this moment, we have an array 
of length $3n$  where each entry is of the form $(e, s, \tau)$ or $\bot$
%; and a 
%real entry of the form $(e, s)$ 
%means that the $e$-th edge has the successor $s$ in the pre-order traversal.
Using oblivious sort, we can move all the $\bot$ entries to the end 
and truncate them away; moreover, the 
remaining real entries are sorted by their edge identifier.
At this moment, we have a resulting array 
of length $2n-1$ where the $i$-th position stores
$(s, \tau)$
where $s$ is the $i$-th edge's successor edge and $\tau$ is its type.

\item 
{\it Weighted list ranking.} 
%\elaine{todo: explain the weighted version}
Invoke an instance of oblivious weighted list ranking, 
such that each edge learns its
distance from the beginning in the list (where distance is defined
as the sum of the weights so far to reach the current edge).


\item  
{\it Send preorder number to vertices.} 
Every edge that is either of type ${\tt LeftChild}$ or ${\tt RightChild}$
gives its number to the vertex the edge travels to.
This can be done through oblivious routing (recall that earlier, every vertex 
already obtained all information from its neighbors, so every vertex
knows the index of the edge coming into itself from the parent).
\end{enumerate}


The above algorithm essentially invokes oblivious weighted list ranking
once and oblivious routing/oblivious sorting $O(1)$ number of times.
The performance overhead is therefore dominated by the list ranking step. 
We thus have the following theorem.

\begin{theorem}[Euler tour for binary tree]
%Assume that $M \geq \log^{1+\epsilon} n$. 
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$. 
Then, we can obliviously realize 
Euler tour on binary trees achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}

\elaine{TODO: maybe we could just suppresse the binary-tree one.}
}

%\subsection{Euler Tour}
\paragraph{Euler tour.} 
%We can extend the above algorithm to trees with unbounded degree.
Suppose that the vertices are %from the range $[n]$. 
numbered $1, 2, \ldots, n$.
The input ${\bf I}$ is an edge list of size $m$, where each entry
in the input array is of the form $(v, w, i)$, denoting
that $w \in [n]$ is the $i$-th child of $v\in [n]$.
%As before, 
We want to output an array $R$ where $R[i]$ stores
vertex $i$'s preorder numbering. 
The $i$-th vertex that 
is reached during a preorder traversal is said to have preorder numbering $i$.
%The algorithm is similar as before:

We can accomplish Euler tour through the following algorithm:

\begin{enumerate}
\item 
{\it Add reverse edges.}
For each edge $(v, w, i) \in {\bf I}$, write down a reverse
edge $(w, v, \bot)$ where $\bot$ denotes that it is a reverse edge going back from $w$
to its parent $v$. 
Let $J$ be the concatenation of ${\bf I}$ and 
all the reverse edges.


\item 
{\it Edge numbering.}
Invoke an instance of all-prefix sum such that all edges 
in ${\bf J}$ acquires a unique index.
Henceforth, we may assume that each 
entry in the input array ${\bf J}$ is of the form $(e, v, w, i)$.
where the additional field $e \in [m]$ denotes the unique index 
of the edge.


\item 
{\it Create successor list.}
Using 
$O(1)$ number of oblivious routings, 
every edge can find and remember its successor edge during
a preorder traversal. \elaine{may need more explanation}
At this moment, obliviously sort the edge list
such that the $i$-th entry stores the $i$-th edge's successor.


\item 
{\it Weighted list ranking.}
Invoke an instance of oblivious weighted list ranking, 
such that each edge learns its
distance from the beginning in the list (where distance is defined
as the sum of the weights so far to reach the current edge).

\item  
{\it Send preorder number to vertices.} 
Every edge that is %either of type ${\tt LeftChild}$ or ${\tt RightChild}$
a forward edge gives its number to the vertex the edge travels to.
This can be done through 2 oblivious routings.
The first oblivious routing allows each of $n$ vertices to learn
the index of the edge coming into itself from its parent.
The second oblivious routing allows 
every vertex to receive its preorder number from this edge.
%(recall that earlier, every vertex 
%already obtained all information from its neighbors, so every vertex
%knows the index of the edge coming into itself).
\end{enumerate}


The above algorithm essentially invokes oblivious weighted list ranking
once and invokes oblivious routing, oblivious sorting, and prefix sum $O(1)$ number of times.
The performance overhead is therefore dominated by the list ranking step. 
We thus have the following theorem.

\begin{theorem}[Euler tour]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$. 
%Assume that $n \geq M \geq \log^{1+\epsilon} n$. 
Then, we can obliviously realize 
Euler tour on unbounded-degree trees achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}

%\subsection{Tree Contraction}

\paragraph{Tree contraction.}
Tree contraction is the following problem:
given a parathesized arithmetic expression expressed as a binary-tree, 
where each leaf stores a number and each internal vertex represents
an operator, evaluate the outcome of the expression. 
We assume that the vertices in the tree are numbered $1, 2, \ldots, n$.
More specifically, the input 
is an array ${\bf I}$ where each entry ${\bf I}[i] = (l, r, {\sf expr})$
where $l \in [n]$ denotes 
the index of the left child of vertex $i\in [n]$, 
$r$ denotes the index of the right child of vertex $i \in [n]$, and 
${\sf expr}$ stores either a number 
or an expression of the form %$a l + b r + c l r + d$
$f(l, r)$ that represents
how to take the two evaluation outcomes at the children $l$ and $r$, and 
evaluate an outcome at the current vertex.
If $l = \bot$ or $r = \bot$, it means that the corresponding child does not exist for
the current vertex.

We can obtain an oblivious tree contraction algorithm 
by modifying the non-oblivious algorithm of \elaine{cite Vijaya's lecture notes} ---
to make it oblivious, the key idea is to 1) rely on oblivious routing
in each iteration for 
parent vertices to receive information from their children in parallel;
and 2) rely on oblivious sorting to remove 
defunct leaves at the end of each iteration.
We describe the detailed algorithm below.
%neighboring vertices
%to fetch information from each other in parallel. 



\begin{mdframed}
Let ${\sf Tree} := {\bf I}$.
Invoke oblivious Euler tour on ${\sf Tree}$, %and the outcome
at the end, each vertex in ${\sf Tree}$ receives its preorder numbering. 
Obliviously sort ${\sf Tree}$ by the vertices' preorder numbering.
At this moment, each entry in ${\sf Tree}$
is of the form ${\sf Tree}[i] = (j, l, r, {\sf expr})$
where $j$ is the $i$-th vertex visited during a preorder traversal,
$l$ and $r$ denote 
$j$'s left and right children respectively, and ${\sf expr}$ denotes an expression.
%is an array ${\sf r}$
%where ${\sf r}[i]$ denotes the preorder numbering of the $i$-th vertex. 
%Using a constant number of oblivious routings,  
%every vertex writes down its immediate parent $p$, and it's grandparent $g$.
%We may now assume that every entry in ${\sf Tree}$ is of the form 
%$(l, r, p, g, {\sf expr})$.
%If $l$, $r$, $p$ or $g$ is $\bot$, it means that the 
%corresponding vertex does not exist.


For $i = 1, 2, \ldots, \ceil{\log_{3/2} n}$:
\begin{itemize}[topsep=1pt,itemsep=1pt]
\item 
Using $O(1)$ number of oblivious routings, every vertex in ${\sf Tree}$ 
receives the information held by both children.

\item 
All vertices in parallel do the following:
if the left child is a leaf and has an odd preorder number, then 
the vertex replaces itself with a shunted vertex (and information of the shunted
vertex can be computed from the two children's information).
\elaine{TODO: explain shunt}

\item 
All vertices in parallel do the following:
if the right child is a leaf and has an odd preorder number, then 
the vertex replaces itself with a shunted vertex (and information of the shunted
vertex can be computed from the two children's information).

\item 
Every vertex in ${\sf Tree}$  
that is a leaf with an odd preorder number 
marks itself as a filler, i.e., effectively deleted. 
Every vertex in ${\sf Tree}$  
that is a leaf with an even preorder number 
divides its preorder number by $2$.

\item 
Obliviously sort ${\sf Tree}$ to remove 
all filler entries to the end, truncate ${\sf Tree}$ preserving 
only the first $\ceil{|{\sf Tree}|/2}$ elements.
%\elaine{truncate array length}
\end{itemize}

Finally, output the expression at ${\sf Tree}[1]$.
\end{mdframed}


The above algorithm begins by invoking oblivious 
Euler tour once and oblivious sorting once; 
afterwards, each of the $O(\log n)$ iterations
invoke oblivious routing and oblivious sort 
$O(1)$ number of times on arrays of exponentially decreasing sizes. 
Thus, it can be implemented in 
$O(\log^2 n \log \log n)$ span, 
$O((n/B) \cdot \log_M n)$ cache complexity, and
$O(n \log n)$ total work.


\begin{theorem}[Tree contraction]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$.
Then, we can obliviously realize 
tree contraction achieving span $O(\log^2 n \log \log n)$,
cache complexity $O((n/B) \log_M n)$, and
total work $O(n \log n)$.
\end{theorem}


\paragraph{Connected components.}
Connected components is the following problem: 
suppose that the vertices are indexed by $[n]$.
The input is an array ${\bf I}$ where each entry 
${\bf I} = (u, v)$ denotes an edge in the graph.
The output is an array ${\bf O}$ where ${\bf O}[i]$
denotes the connected component vertex $i \in [n]$
belong to. It should be the case that all vertices belonging to
the same connected component 
receive the same number in the output array.

We describe a cache-agnostic, oblivious algorithm for accomplishing 
connected components. 
Our algorithm follows the blue-print of Shiloach 
and Vishkin~\cite{vishkinCC}, but we realize the communication steps
between vertices and edges.
At a very high level, in their algorithm, a core data structure 
is a parent-pointer graph: every vertex $v$ stores 
their current parent henceforth denoted $p(v)$, and updates its pointer throughout the algorithm.
At the end of the algorithm, the parent-pointer
graph is guaranteed to produce one star per connected component
where every vertex in the same connected component points to 
a ``root'' of the connected component, where the root is the representative
of the connected component. 
The root's index will become 
the connected component's identifier
assigned to the vertices belonging to this connected component.

Initially, all vertices point to themselves.
Now, 
Shiloach and Vishkin's algorithm~\cite{vishkinCC}
proceeds in $O(\log n)$ iterations, and during each iteration,
the following actions take place:
\begin{itemize} 
\item 
{\it Shortcutting}: every vertex %might decide to connect to its 2-hop parent.
in parallel updates its parent pointer to its grandparent, i.e., $p(v) \leftarrow p(p(v))$, 
if the grandparent is different
from the parent. Moreover, the new parent gets notified that some new vertex
has pointed to it. 

\item  {\it Conditional hooking.}
%If a vertex $v$'s did not update its parent the earlier step, and 
%the parent $p(v)$ has a greater index than 
%$v$'s neighbor's parent, 
If a vertex $v$'s parent $p(v)$ did not receive any new children in the previous step
(i.e., $v$ is in a star at the beginning of this iteration), 
then update 
$p(v)$'s pointer to point to 
a neighbor's parent which is smaller, i.e., 
if $(u, v)$ is an edge in the graph, $p(u) < p(v)$, and moreover $p(v)$ was not
updated in the earlier step, then update
$p(p(v)) \leftarrow p(u)$ --- if multiple such updates are made
to $p(v)$, an arbitrary one of them will succeed; moreover,
this vertex who got hooked onto will  get notified that some vertex
has newly pointed to it.

\item  {\it Unconditional hooking.}
%The root of a tree (i.e., the vertex's parent is itself) 
%is said to be stagnant if it did not get any new children, or hook onto a new parent so far
%during this iteration.
If a vertex $v$'s parent $p(v)$ did not receive any new children so far in this  
iteration (i.e., the vertex is in a star at the beginning of the iteration), 
%If a vertex $v$'s parent is a stagnant root, 
and moreover, the vertex
$v$ has a neighbor $u$ in the graph such that $p(u) \neq p(v)$, then 
update $p(p(v)) \leftarrow p(u)$. If multiple such neighbors exist, choose an arbitrary one's
parent to hook onto.
%the corresponding tree 
%is called a stagnant tree.

%\item 
%{\it Second shortcutting.}
%Repeat the shortcutting step mentioned above.
\end{itemize} 

To implement their algorithm obliviously, it suffices to show how to 
accomplish the following communication primitives obliviously:
\begin{enumerate}[itemsep=1pt,topsep=1pt]
\item 
For each vertex to in parallel receive information from its parent. %(or grandparent resp.).
This is needed for the vertex to %decide whether to shortcut to the grandparent.
find out who its grandparent is during the shortcutting steps. 
%, and decide whether to shortcut to the grandparent. 

\item 
For each vertex to 
in parallel  aggregate information from all of its 
neighbors in the original graph, or from its children in the parent-pointer graph. 
This is needed for each vertex to find out if there is a neighboring tree
for its parent to hook onto, and is needed for the root 
to learn which other tree to hook onto.
This is also needed for a vertex to learn %if it is stagnant.
if any new vertex has newly pointed 
to itself.
\end{enumerate}

To realize the above steps, our algorithm is partly 
inspired by Nayak et al.~\cite{graphsc} who
studied oblivious algorithms in an EREW PRAM model.
Imagine that our algorithm maintains a joint edge/vertex list denoted $L$
containing two types of entries.
Each vertex entry stores 
a vertex's index, its parent pointer, and 
additional information gained during in the algorithm 
(e.g., the parent of some neighbor, the iteration in which the vertex's parent
was last updated, and the iteration in which the vertex last received new children).
Each 
edge entry stores an edge in the original graph.
Moreover, the undirected edge
$(u, v)$ appears twice, once as $(u, v)$ and 
the other times as $(v, u)$. 
\ignore{
\begin{itemize}
\item 
{\it Vertex entry:}
there are $n$ vertex entries, each of the form $({\tt vertex}, i, p, {\sf payload})$
where ${\tt vertex}$ denotes the type of the entry,
$i \in [n]$ 
denotes the vertex's index, $p$ denotes its parent, and ${\sf payload}$
stores 
additional information gained during in the algorithm (e.g., the parent of some neighbor $u$).  

\item 
{\it Edges in the original graph:}
The list also contains all the $m$ edges in the original graph,
where each undirected edge 
$(u, v)$ appears twice, once as $({\tt edge}, u, v)$ and 
the other times as $({\tt edge}, v, u)$. %\elaine{is this needed}
\end{itemize}
}
Observe that the length of the list $L$ is $n + 2m$
where $n$ denotes the number of vertices and $m$ denotes the number of edges
in the original graph.
\elaine{say somewhere that we leak only n and m for all the graph algorithms}


Now, type-1 communication where each vertex receives information from the parent can be 
realized
through oblivious routing, where every vertex-entry 
in $L$ wants to fetch the entry identified by the parent's index.
Type-2 communication 
can be implemented through a combination of oblivious sorting and oblivious aggregation.
Suppose that each vertex wants to aggregate information from each neighbor
in the original graph.
This can be accomplished as follows: 
obliviously sort the array $L$ such that for each vertex $v \in [n]$,
the unique vertex
entry for $v$ appears first, followed by all edges $(v, *)$.
Now, run 
an oblivious aggregation algorithm for each 
vertex to  
aggregate information from all of its neighbors.

For a parent to aggregate information from all of its children
is similar but slightly more complicated:
notice that every vertex entry also stores an edge in the 
parent-pointer graph.
To perform the aggregation, each vertex entry must first  
replicate itself into two entries, one serves
as a vertex and the other serves as an edge --- moreover, this must
be done in a way that preserves obliviousness: 
\begin{itemize}
\item 
First, rely on oblivious sorting so all $n$ vertex
entries appear in the front of $L$.
Now, the first $n$ entries in $L$ replicates a temporary copy of itself which
represents an edge in the parent-pointer graph.
At this moment, the array $L$ is temporarily expanded to a length of $2 n + 2m$.

\item 
Obliviously sort the expanded list $L$ 
such that every vertex $v$ appears immediately in front of
all edges going into $v$ in the parent-pointer graph.
\item 
Use oblivious aggregation for all vertices to aggregate information from their children
in the parent-pointer graph.
\item 
Finally, use oblivious sorting to move all temporary copies
of vertex entries created above to the end of the array,  
and truncate those entries away. The resulting array would again be $n + 2m$ in size.
\end{itemize}


Using the above algorithms to implement the parallel communication
steps in Shiloach and Vishkin~\cite{vishkinCC},
we obtain a cach-agnostic, oblivious algorithm for connected components
as stated in the following theorem:

\begin{theorem}[Connected component]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$, and let $m$
denote the number of edges in the graph.
Then, we can obliviously realize 
connected component achieving span $O(\log^2 m \log \log m)$,
cache complexity $O((m/B) \log_M m \log m)$, and
total work $O(m \log^2 m)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}


\paragraph{Minimum spanning forest.}
The input is an edge array ${\bf I}$ where each entry ${\bf I}[i] = (u, v, w)$
stores an edge of the graph $(u, v)$ and it weight $w \geq 0$.
We may assume that all vertices have indices from the range $[n]$.
The output is a bit array ${\bf O}$
where ${\bf O}[i] = 1$ 
means that the $i$-th edge in the input array is in the minimum-weight spanning forest.

Minimum spanning forest can be computed using a very similar algorithm 
as the aforementioned connected components algorithm. 
%The only difference is that during each of the $O(\log n)$ iterations, nodes 
Initially, everyone's parent pointer points to itself.
Next, repeat the following for $O(\log n)$ iterations:
\begin{itemize}
\item {\it Shortcutting.}
Same as before.
\item  {\it Conditional hooking.}
%If a vertex $v$'s did not update its parent the earlier step, %and $v$ is in a star, 
For a vertex $v$, if 
$p(v)$ did not receive 
any new children in the previous step (i.e., the vertex was in a star
at the beginning of this iteration), 
then let $S$ be the set of $v$'s neighbors in the original graph 
such that for $u \in S$,
$p(u) \neq p(v)$.
Find the $u^* \in S$ 
whose edge weight is the minimum, 
and send $((v, u^*), w^*, p(u^*))$
to its parent $p(v)$ where $w^*$ is the weight of the edge $(v, u^*)$.

Every vertex $z$ that is a root (i.e., its parent pointer is itself)
looks at all the tuple it has received, 
choose the one with the minimum edge weight, say $((v', u'), w', p(u'))$, 
if $p(u') < p(z)$,  
 set $p(z) := p(u')$, and record that the edge $(v', u')$ is in the  minimum spanning forest.

\item  {\it Unconditional hooking.}
%The definition of a stagnant root is the same as before.
If a vertex $v$'s parent $p(v)$ %is a stagnant root, 
did not receive any new children so far in this iteration, 
let $S$ be the set of $v$'s neighbors in the original graph 
such that for $u \in S$,
$p(u) \neq p(v)$. 
Find the $u^* \in S$ whose edge weight is the minimum, 
and send $((v, u^*), w^*, p(u^*))$ to $p(v)$ if $S$ is not empty.
%and send $((v, u^*), w^*, p(u^*))$
%to its parent $p(v)$ where $w^*$ is the weight of the edge $(v, u^*)$.

Every vertex $z$ that is a stagnant root 
looks at all the tuple it has received, 
choose the one with the minimum edge weight, say $((v', u'), w', p(u'))$, 
set $p(z) := p(u')$, and record that the edge $(v', u')$ is in the  minimum spanning forest.

%\item {\it Second shortcutting.}
%Same as before.
\end{itemize}



To implement this algorithm, we can use the same techniques
as in connected components 
to implement the communication 
among neighbors (either in the original graph or in the parent-pointer graph) in each 
iteration.
The only 
additional communication is necessary is to record any edge 
chosen. This
can be accomplished through oblivious routing.

\begin{theorem}[Minimum spanning forest]
Assume that $M \geq \log^{1+\epsilon} n$ and that $n \geq M \geq B^2$, and let $m$
denote the number of edges in the graph.
Then, we can obliviously realize 
minimum spanning forest achieving span $O(\log^2 m \log \log m)$,
cache complexity $O((m/B) \log_M m \log m)$, and
total work $O(m \log^2 m)$.
Moreover, the algorithm is cache-agnostic.
\end{theorem}






==> bldgblock.tex <==
\section{{\sc Butterfly-Random-Permute} and {\sc Butterfly-Sort}: Details}
\label{sec:rec}


%\section{Details of Our Meta-Algorithm for Sorting}

\subsection{Preliminary: Oblivious Bin Placement}
\label{sec:warmup}

\ignore{
In this section, we provide additional details of our ``meta-algorithm''.
This meta-algorithm obliviously sorts $n$ input elements 
with $O(n \log n)$ total work, 
but it does not worry about being cache efficient or 
having small span.
Our full construction later (Section~\ref{sec:rec})  
is a novel way to implement this meta-algorithm, achieving  
small cache complexity and span.
}


%\subsection{Bin Placement}
\label{sec:obp}

We consider the problem of obliviously placing the elements in one layer in %the {\sc Meta-ORBA}
our ORBA
algorithm into their designated bin in the next layer. For this, we
 will need a data-oblivious building block called {\it bin placement} that places  
elements into their desired bins, and pads each 
bin with filler elements to its capacity.
In {\sc Meta-ORBA} and {\sc Rec-ORBA}, we will  
use data-oblivious bin placement %to route elements to bins
for small problem instances of size $\log^3 n$ (where $n$ is
the size of the array we want to sort). 


Bin placement %is the following primitive~\cite{circuitopram}.
realizes the following deterministic functionality~\cite{circuitopram}.
Let $\bins$ denote the number of bins, and let $Z$ denote the target bin capacity.
We are given an input array 
denoted ${\bf I}$, where 
each element is either a {\it filler} denoted $\bot$ or a {\it real} element
that is tagged with a bin identifier ${\group} \in [\bins]$ denoting which bin 
it wants to go to.
It is promised that every bin will receive at most $Z$ elements.
Now, move each real element in ${\bf I}$ to 
its desired bin.
  If any bin is not full after the real elements have been placed, pad it with filler elements {\it at the end}
to a capacity of $Z$. Output the concatenation of the $\bins$ bins as a single array.
%
An algorithm that obliviously realizes bin placement by Definition~\ref{defn:obl} 
is called oblivious bin placement.



Chan and Shi~\cite{circuitopram} described a deterministic, data-oblivious algorithm 
that accomplishes bin placement 
in total work $O(\widetilde{n} \log \widetilde{n})$
and parallel runtime $O(\log \widetilde{n})$ where $\widetilde{n} = \max(|{\bf I}|, \bins \cdot Z)$
on a
CREW PRAM. Thus the algorithm has 
span 
$O(\log^2 \tilde{n})$ in a binary fork-join model.
More specifically, Chan and Shi's algorithm~\cite{circuitopram}
invokes the AKS sorting network~\cite{aks} $O(1)$
number of times on arrays of length at most $\widetilde{n}$.
We will use bin placement in {\sc Meta-ORBA}, so for completeness, we give a brief description of Chan and Shi's 
data-oblivious bin placement algorithm which relies on $O(1)$ number of oblivious sorts (which can be instantiated
with the AKS sorting network~\cite{aks}):


\paragraph{Bin Placement Algorithm.} 


\begin{enumerate}[leftmargin=5mm,itemsep=1pt]
\item 
For each group ${\group} \in [\bins]$,
append $Z$ temporary elements of the form $({\tt temp}, {\group})$
to the resulting array.
At this moment, all real elements and ${\tt temp}$ elements
are tagged with ${\group}$ which is called the element's group number.
These {\tt temp} elements ensure that 
every group will receive at least $Z$ elements after the next step\footnote{The {\tt temp}
elements are placeholder elements that make sure each array must be fully filled. 
They are not the same as the filler elements that might be part of the input array ${\bf I}$.
Both real elements and {\tt temp} elements are assigned group numbers, but filler
elements do not have group numbers.}.


\item
Obliviously sort the resulting array by 
the group number, placing all
  fillers at the end.
When elements have the same group number, 
%place elements with higher priority 
%in the front, and 
place {\tt temp} elements after real elements.

\item 
Each element in the array finds 
the leftmost element in its own group by invoking oblivious propagation. 
Now for each element in the array in parallel, 
if its offset within its own group is greater than $Z$, 
assign it with the tag ${\tt excess}$; 
otherwise, assign it with the tag ${\tt normal}$.


\item 
Obliviously sort the 
resulting array placing all elements tagged with ${\tt excess}$ 
and all filler elements at the end; 
and all other elements should 
be ordered by their group number.


\item 
Truncate the resulting array
keeping only the first $\bins \cdot Z$ elements --- the resulting array is called ${\bf O}$.

\item 
For every element in ${\bf O}$: if it is a {\tt temp} element, replace with a filler; 
further, remove 
tags such as {\tt excess} and {\tt normal} that are needed only internally 
by this algorithm.
Output ${\bf O}$.
\end{enumerate}

%\paragraph{Analysis.}


\ignore{
\subsection{{\sc Meta-ORBA}: Random Bin Assignment}

Random bin assignment is an algorithm that realizes the following randomized functionality.
Let %$Z = \omega(\log \kappa)$ 
$Z$ be an even integer. 
Upon receiving an input array with $n := \bins \cdot Z/2$ real elements,  
assign each element to a {\it random }
bin among a total of $\bins$ output bins.
Finally, for each output bin, if it receives fewer than $Z$ elements, pad
the bin {\it at the end} with {\it filler} elements to a capacity of exactly $Z$;
if it receives more than $Z$ elements, 
truncate the bin to a capacity of $Z$.
Output the list of $\bins$ output bins. 
An algorithm 
that obliviously realizes random bin assignment
by Definition~\ref{defn:obl}
(see Section~\ref{sec:d-o})
is called {\it oblivious random bin assignment} (ORBA).
Observe that by the requirements of Definition~\ref{defn:obl}, 
the algorithm's access patterns cannot reveal the random bin choices 
made by each element (except for a small $\delta$ failure probability).


\paragraph{Algorithm.}
Below we describe our meta-algorithm for accomplishing ORBA, called {\sc Meta-ORBA}. 
Let the bin size $Z = \log^2 n$, and let $\gamma$ 
be a branching factor which is assumed to be a power of $2$.
Our {\sc Meta-ORBA} algorithm will invoke instances of 
the oblivious bin placement algorithm (see Section~\ref{sec:obp}) 
to plaze $\gamma \cdot Z$ elements into $\gamma$ bins.
Henceforth we use the notation 
$${\bf O}_0, \ldots, {\bf O}_{\gamma-1}  
\leftarrow {\sf BinPlace}({\bf I}_0, \ldots {\bf I}_{\gamma-1}, s)$$
to mean the following:
given an input list consisting of $\gamma$ bins 
denoted ${\bf I}_0, \ldots {\bf I}_{\gamma-1}$ each of size $Z$, 
using the algorithm in Section~\ref{sec:obp}, 
obliviously place the elements into 
$\gamma$ output bins denoted ${\bf O}_0, \ldots, {\bf O}_{\gamma-1}$, each also of capacity $Z$;
moreover, to decide which bin each element falls into, we use 
the bits indexed $s+1, s+2, \ldots, s+\log_2 \gamma$
in the elements' random labels (where we assume that the first bit is indexed with $1$).

%for small instances 
%of size $\gamma \cdot Z$.

\ignore{
\begin{figure*}
\begin{center}
\includegraphics[width=0.6\textwidth]{RadixBucketSort1}
\end{center}
\caption{An illustration %of the {\sc Meta-ORBA} algorithm 
by Asharov et al.~\cite{bucketosort} for the special
case $\gamma = 2$. Our {\sc Meta-ORBA} algorithm 
achieves a $\log \log n$ factor improvement in parallel runtime relative
to Asharov et al.~\cite{bucketosort} by adopting
$\gamma = \Theta(\log n)$.}
\label{fig:orba}
\end{figure*}
}

\begin{mdframed}
\begin{center}
${\text{\sc Meta-ORBA}}^\gamma({\bf I})$
\end{center}
\noindent{\bf Input:} 
we assume that $n = |{\bf I}| = \bins \cdot Z/2$
%the input ${\bf I}$ is an array containing $n := \bins \cdot Z/2$ elements
where $\bins$ is a power of $2$.

\vspace{5pt}
\noindent{\bf Algorithm:}

First, assign each element 
in ${\bf I}$ with a {\it random label} of $\log_2 \bins$ bits.
View the input ${\bf I}$
as a set of $\bins$ bins each with $Z/2$ elements. Pad each bin with {\it filler}
elements to a capacity of $Z$.
Let $A_{0}^{(0)}, A_{1}^{(0)}, \ldots, A_{\bins-1}^{(0)}$
denote the list of $\bins$ initial bins.

%\elaine{check off by 1}
For $i = 0$ to $\log_\gamma \bins - 1$:

\vspace{-10pt}
\begin{itemize}[topsep=0pt,itemsep=0pt,leftmargin=5mm]
\item[] 
For $j = 0$ to $\bins/\gamma - 1$: 
\begin{itemize}[topsep=0pt,itemsep=0pt,leftmargin=5mm]
\item[] 
let $j' = \lfloor j/\gamma^i \rfloor \cdot \gamma^{i+1}$, \\[3pt]
 ${A}_{\gamma j}^{(i+1)}, {A}_{\gamma j + 1}^{(i+1)}, \ldots,  
{A}_{\gamma (j +1)-1}^{(i+1)}\leftarrow 
{\sf BinPlace}(\{{A}_{j' + j + k \cdot \gamma^i}^{(i)}\}_{k \in \{0, 1, \ldots, \gamma-1\}},
%,  {A}_{j' + j + \gamma^i}^{(i)},  
% {A}_{j' + j + 2 \gamma^i}^{(i)}, \ldots, 
% {A}_{j' + j + (\gamma - 1)\gamma^i}^{(i)}, 
\log_2 \gamma \cdot i)$
%\newline
\end{itemize}

\end{itemize}

Output $A_0^{(\log_\gamma \bins)}, \ldots, A_{\bins-1}^{(\log_\gamma \bins)}$.
\end{mdframed}


Our algorithm is based on the earlier works 
of Asharov et al.~\cite{bucketosort} and Chan et al.~\cite{cacheoblosort}.
Their algorithm can be viewed as a special case of ours where $\gamma = 2$;
%(see also Figure~\ref{fig:orba});
however, their algorithm is a $\log \log n$ factor away from optimal on a
%VLR: Check if CREW or EREW. If not sure just say PRAM
CREW PRAM 
as explained below.
In their algorithm, the for-loop on $i$ will repeat $\Theta(\log n)$ iterations.
In each iteration $i$, 
they take pairs of bins which contain elements whose first $i-1$ bits 
of their labels already agree. They then look at the 
$i$-th bit of their labels, 
and based on its value, 
they assign each element in the input pair of bins into 
one of two output bins.
Therefore, each iteration must invoke 
an instance of two-way bin assignment for every small problem of size 
$2 Z$, and there are $\bins/2$ such instances.
The two-way bin assignment can be realized with either a sorting network
such as AKS~\cite{aks} which can sort $m$ elements in $O(m \log m)$ work
and $O(\log m)$ parallel runtime, or an
oblivious tight compaction algorithm~\cite{optorama,paracompact}
which can sort $m$ elements tagged with 0/1 keys  
in $O(m)$ work and $O(\log m)$ parallel runtime on a
%VLR: Check if CREW or EREW. If not sure just say PRAM
CREW PRAM.
If AKS is adopted for the two-way bin assignment, 
the total work of the resulting ORBA would be
$O(n \log n \log \log n)$, and the parallel runtime  
on an EREW PRAM would be $O(\log n \log \log n)$.
If an oblivious tight compaction algorithm 
is adopted, the resulting ORBA would have  
$O(n \log n)$ total work but still 
$O(\log n \log \log n)$ parallel runtime on an EREW PRAM.


Our new idea is to generalize the prior works~\cite{bucketosort,cacheoblosort}
with a more general branching factor $\gamma$.
In other words, in every iteration $i$, we take $\gamma$-tuples of bins
in which the elements already agree on the first 
$\log_2 \gamma \cdot (i-1)$  
of their labels, 
we then look at the next 
unconsumed  $\log_2\gamma$ bits of the elements labels and classify elements in the  
$\gamma$ input bins to $\gamma$ output bins.
To make this generalization work, 
%we cannot directly use AKS to make the $\gamma$-way bin assignment.
we will need to employ the oblivious bin placement algorithm 
described in Section~\ref{sec:obp}
to perform a $\gamma$-way bin assignment (as opposed to $2$-way).

With this generalization, and by setting $\gamma = \Theta(\log n)$, 
we can save an extra $\log \log n$ factor in the parallel runtime in comparison with 
the prior works~\cite{bucketosort,cacheoblosort} (assuming that oblivious tight compaction
is used to instantiate their 2-way bin assignment).
Specifically, we achieve $O(n \log n)$ total work and $O(\log n)$
parallel runtime on an EREW PRAM.

\paragraph{Overflow analysis.}
Our {\sc Meta-ORBA} algorithm has deterministic data access patterns
that are independent of the input ${\bf I}$.
However, if some bin overflows its capacity, the algorithm can lose real elements  
during the routing process.
Asharov et al.~\cite{bucketosort}
and Chan et al.~\cite{cacheoblosort} proved that for the special case $\gamma = 2$, 
the probability of overflow is upper bounded by $\exp(-\Omega(\log^2 n))$
assuming that the bin size $Z = \log^2 n$.
It is not hard to see that their argument works for general choices of $\gamma$ too, as we argue now:
Suppose that $\gamma = 2^r$, then  
the elements %destined for each of the iteration-$i$ output bins
in the level-$i$ bins\footnote{A bin in {\it level} $i$ is denoted
$A_{*}^{(i)}$ in the {\sc Meta-ORBA} algorithm description.}  
in our ${\text{\sc Meta-ORBA}}^{\gamma = 2^r}$ correspond exactly to the elements 
in the level-$(r \cdot i)$ bins in ${\text{\sc Meta-ORBA}}^{\gamma = 2}$.
Since the failure probability $\exp(-\Omega(\log^2 n))$
is negligibly small in $n$, we have the following theorem:

\begin{theorem}
Let $Z = \log^2 n$ and $\gamma = \Theta(\log n)$ in the above ${\text{\sc Meta-ORBA}}^\gamma$
algorithm. Then the algorithm ${\text{\sc Meta-ORBA}}^\gamma$ obliviously realizes random bin assignment 
on an EREW PRAM with $O(n \log n)$ 
total work and $O(\log n)$ parallel runtime.
\end{theorem}

\subsection{Random Permutation}
\label{sec:orp}

Random permutation is the randomized 
functionality that takes an input array ${\bf I}$ and outputs
a random permutation of ${\bf I}$.
An algorithm that obliviously realizes random permutation by Definition~\ref{defn:obl} is called
oblivious random permutation (ORP).
Observe that by the requirements of Definition~\ref{defn:obl}, 
the algorithm's access patterns cannot reveal the random permutation 
that is being applied to the input (except for a small $\delta$ failure probability).


The prior works by Asharov et al.~\cite{bucketosort}
and Chan et al.~\cite{cacheoblosort}
showed that we can rely on an ORBA to construct an ORP as follows:
\begin{enumerate}[leftmargin=5mm,itemsep=1pt]
\item 
Let ${\bf I}$ be an input array containing $n = \bins \cdot Z/2$ elements 
where $\bins$ is assumed to be a power of $2$.
\item 
Invoke an instance of {\sc Meta-ORBA} 
to place each input element into a randomly chosen bin among a total of $\bins$ bins,
where each bin is padded with filler  
elements to a capacity of $Z$.

\item 
At this moment, for each of the $\bins$ bins, 
apply a na\"ive oblivious random permutation to permute within the bin.
This can be accomplished by assigning each
real and filler element a $\log n \log \log n$-bit
label, and obliviously sorting the elements in the bin based on their keys.
It is not hard to see that the probability of 
having label collision is negligibly small in $n$.

\item 
\label{step:last}
Finally, we remove all filler elements from all the bins ---
this step need not be oblivious, and can be computed with a prefix sum computation.
\end{enumerate}

In the last step of the above algorithm, the actual load of  
each final bin is revealed ({\it c.f.}, it is important that one 
does {\it not} leak the actual loads
of the intermediate bins in the butterfly network).
As Asharov et al.~\cite{bucketosort}
and Chan et al.~\cite{cacheoblosort} argue, the loads of 
the bins are simulatable with knowledge only of the length
of the input array ${\bf I}$ and the bin size $Z$ but not of the actual contents of ${\bf I}$.
For this reason, the above algorithm is proven
to obliviously realize random permutation 
by Asharov et al.~\cite{bucketosort}
and Chan et al.~\cite{cacheoblosort}.
Note also, the random labels must each be super-logarithmic in length to 
guarantee that no collision happens except with negligible probability, such that the resulting 
permutation has negligible statistical distance from a random one. 

%\vlr{Elaine, small wording changes.}
%looks good
This
ORP algorithm runs with 
$O(n \log n)$
total work and $O(\log n)$ parallel runtime on an 
EREW PRAM since the costs are dominated by {\sc Meta-ORBA}.

\subsection{Constructing Oblivious Sort from ORP and Non-Oblivious Sort}

Asharov et al.~\cite{bucketosort} and Chan et al.~\cite{cacheoblosort}
proved that given an ORP, one can construct an oblivious sorting algorithm
by first running ORP to randomly permute the input array, and then
applying any {\it comparison-based} non-oblivious sorting algorithm to sort
the permuted array. 
It is important that the non-oblivious sorting algorithm adopted
be {\it comparison-based}, otherwise the resulting algorithm 
may leak information through its access patterns (e.g., a non-comparison-based
sorting algorithm can look at some bits in each element and place
it in a corresponding bin).

}





==> oldsort.tex <==

\section{Sorting a Random Input: {\sc Rec-Sort}}

%\vlr{I need to go to early voting which ends today. I haven't proofed this, and will get back to it in an hour's time. Feel free to review this in the meantime, and make your updates/comments.}

Earlier, we relied on an oblivious random permutation  
to permute the input array, and 
then we could sort the array using any non-oblivious, comparison-based
sorting algorithm (specifically, we used the SPMS algorithm~\cite{CR17} 
as the non-oblivious sorting algorithm).

\elaine{Vijaya: i changed the name to Rec-Sort because this algorithm need not be oblivious, it is to replace 
SPMS which is non-oblivious too}

We now describe a new, conceptually simple 
comparison-based sorting algorithm 
that can sort {\it randomly permuted input arrays}. %with all but negligible probability. 
%algorithm called {\sc Rec-Sort} to sort 
%a randomly permuted input array. 
Our new algorithm has slightly higher span than SPMS~\cite{CR17} 
but it is conceptually much simpler --- notably, it relies
on the same butterfly network structure as {\sc Rec-ORBA}.
With {\sc Rec-ORBA} and {\sc Rec-Sort}, we could construct
a full-blown, conceptually simple oblivious sorting algorithm, by first randomly permuting
the input array obliviously using {\sc Rec-ORBA} as a core building 
block; and then relying on {\sc Rec-Sort} to sort the permuted array.
\ignore{
Here we consider the problem of sorting a random permutation of the input elements contained in an array ${\bf I}[1..n]$,  \elaine{Vijaya: i changed the array name to I, since B is block size}
data-obliviously with cache-efficiency and high parallelism. Our overall sorting algorithm is
obtained by running {\sc Rec-ORBA} on the given input and then generating the randomly permuted
array ${\bf I}$. We continue to call this preceding algorithm {\sc Rec-ORBA}. Our algorithm is based on sample sort,  where we initially pick pivots that will use in a staggered
fashion through the algorithm. 
}

As mentioned, {\sc Rec-Sort}
uses the same network structure as {\sc Rec-ORBA},
Initially, elements in the input array ${\bf I}$ are partitioned
in bins containing $\log^2 n$ elements each.  %We assume that the number of bins is a power of 2.
Then, the elements traverse
a $\log n$-way butterfly network: at each step, we use AKS 
to distribute a collection of $\log n$ bins at the previous level
into $\log n$ bins at the next level. 
The distribution uses 
pre-selected pivots 
to decide which bin each element goes to.
Earlier in {\sc Rec-ORBA}, we needed to use filler elements
to hide the actual load of each bin, %but since the input has already
but we do not need filler elements in {\sc Rec-Sort}
since the algorithm need not be data-oblivious.
%As noted above, {\sc Rec-Sort} uses exactly the same algorithm as {\sc Rec-ORBA}, but at each level the output of the AKS sorter for
%the elements from the $\log n$ bins in the previous level are distributed across $\log n$ bins
%in the next level using suitable pivot elements that are chosen at the start of the algorithm. 
The pivots
are chosen in a pre-processing phase, 
so that we can guarantee that every bin has $O(\log^2 n)$ elements with all but negligible
failure probability, as we show below.

\elaine{TODO: make a pass over vlr.tex, introduce terms like logn-way butterfly network there}


\ignore{
We first describe the {\sc Rec-Sort} algorithm 
using the AKS algorithm to sort the pivots and then discuss the
changes to the bounds if we use bitonic sort in place of AKS.

Our algorithm {\sc Rec-Sort} has the same structure as {\sc Rec-ORBA}, and the elements in $B$ are initially partitioned
in bins containing $\log^2 n$ elements each. We do not need filler elements for {\sc Rec-Sort} if the 
input is generated by  {\sc Rec-ORBA} but we could use filler elements, which would make {\sc Rec-Sort}
a stand-alone oblivious sorting algorithm which has good performance bounds for random inputs.
}
%\vlr{Elaine, is the above statement correct? It's correct for the algorithm, but I'm not sure about the pivots.}

The initial step in {\sc Rec-Sort} is to generate a sample $\Pi$ of size close to $n/\log n$ from
the input array ${\bf I}$ 
by sampling each element with probability $1/\log n$. We then sort $\Pi$ using AKS
(and we shall later describe a practical variant that uses bitonic to sort the samples). 
Using AKS this
can be performed with optimal cache complexity %$O((n/B) \cdot \log_M n)$ and 
$O(n/B)$ \elaine{i changed this expression to n/B} and 
$O(\log^2 n)$ span
with binary fork-joins. 
%(we discuss small 
%modifications to the algorithm if we replace AKS with bitonic sort in order to obtain a very simple algorithm).
This is the step that dominates our span. We then pick every $(\log^2 n)$-th element in the sorted
$\Pi$ to obtain our set of $\approx n/\log^3 n$ pivots in sorted order. We then re-order these pivots
with another AKS sort so that pivots for each subproblem of 
$\log n$ bins are in contiguous locations. This
can be done as follows, where ``level'' refers to %the non-recursive version of our ORBA algorithm, which we
a level in our ORBA meta-algorithm henceforth called {\sc Meta-ORBA}
(i.e., the non-recursive version). 
\elaine{Vijaya: i am calling this a meta algorithm later, so let's call it Meta-ORBA, introduce
this term Meta-ORBA earlier in vlr.tex}


{\sc Pivot Selection}

1. Pick a random set $\Pi$ of about $n/\log n$ pivots by sampling each element with probability $1/\log n$.

2. Let $\ell = \log^3 n$ and $r= n/\ell$. Sort $\Pi$ and move every $\log^2 n$-th element in sorted order into a new sorted array $s[1 .. r]$. 
\elaine{Vijaya: i am bothered that this calls another complicated
sorting algorithm like 
AKS, why is this better than calling SPMS? maybe we should describe it only with bitonic
and skip the AKS}

\elaine{Vijaya: i don't think it's very precise here. 
the number of samples you pick is a random variable. 
if you pick a fixed number of pivots, the last segment's size could have large deviation}

3. The elements in positions $j/\log n$, $1\leq j \leq \log n$ in array $s$ are the pivots for the first level of {\sc Meta-ORBA}.
Between each successive pair of first-level pivots are 
 $\log n$ evenly-spaced pivots for the second level (so there are $\log^2 n$ pivots for the second level), and so on. 

 Label each pivot element as $(i,j,value)$ where $i$ is the level in which it is a pivot, and $j$ is the subproblem on the $i$-th level in which it
 is a pivot. 
 
 4. Sort the pivots by their labels, so that the pivots are now in sequenced in sorted order, level by level, and within each level, in sorted order by subproblem, in within each subproblem, in sorted order by value.
 
 \vone
 Using the pivots to orchestrate the sorting of the elements into bins, as in {\sc Rec-ORBA}:
 
 
 \vone
 {\sc Rec-Sort}$({\bf I}[1..n])$
 
 Initially group the elements into $\bins = n/\log^3 n$ bins, each containing $\log^2 n$ elements.
 Then,
 
  (a)  group the bins into $\sqrt{\bins}$ groups of $\sqrt \bins$ bins each, and recursively sort each group using the precomputed pivots for the level corresponding to groups of $\sqrt \bins$ bins. 
  
  (b) As in {\sc Rec-ORBA}, perform a transpose on the bins so that all bins separated 
\elaine{Vijaya: i don't understand the usage of the word separated, do you mean that
the elements in the bin must be sandwiched
in between two pivots?}
by the same pair
  of pivots are placed next to each other. 
  
  (c) group the bins into $\sqrt{\bins}$ groups of $\sqrt \bins$ bins each, and recursively sort the elements in each group using the precomputed pivots for the level corresponding to groups of $\sqrt \bins$ bins 
  (the levels in the second recursive call with start around  $i= \frac{\log  n}{2\log\log n}$).

 \vone
 
 The base case occurs when the number of bins reduces to $\log n$ at which point the
 $\Theta (\log^3 n)$ elements in these $\log n$ bins are sorted using the AKS network
 using the precomputed set of pivots for  this group.  The exact set of pivots to use can be determined  by including the range of levels and subproblems  in the calling
  sub-problem. 
\elaine{Vijaya: i cannot parse the above sentence}
For example the range for the call to the first recursive sub-problem of size 
  $\sqrt{\beta}$ is $([1 .. \log n/2\log\log n], [1 .. \sqrt\beta/\log n])$.
 
 \vone
 {\bf Analysis.}  Since we are binning the elements using the pivots and sorting using AKS at the base,
 this is a correct sorting algorithm. It remains to establish bounds on the performance of this algorithm
 when given a randomly permuted input.
 
 
 It is readily seen that by over-sampling and then using every $\log^2 n$-th element in the sorted sequence $\Pi$ 
 as a pivot, the number of elements in array ${\bf I}$ that have ranks between two
 successive pivots is at most  $\log^3 n + o(\log^3 n)$ with negligible failure probability. In fact, we
  now show the number of elements placed in any bin is $O(\log^2 n)$ with 
all but negligible probability of failure.

 
Like {\sc Meta-ORBA}, the non-recursive
version of {\sc Rec-Sort}
is the meta-algorithm called {\sc Meta-Sort}.
{\sc Rec-Sort} is an cache-efficient implementation of {\sc Meta-Sort}
in a binary-forking model.
 Consider a collection of $\log n$ bins in the $j$-th subproblem in level $i-1$ of {\sc Meta-Sort}
 whose contents are input to an AKS sorter. Let us refer to this as group $(i-1,j)$. These elements will be 
 distributed to $\log n$ bins in level $i$ using the $\log n$ pivots with label pair $(i-1,j)$.
 The elements in these $\log n$ bins in group $(i-1,j)$ came from $\log^{i-1} n$  groups of 
 $\log n$ bins  in the first level,
 each containing exactly $\log^2 n$ elements from input array ${\bf I}$. Let $U$ be the set of elements in
 these $\log^{i-1} n$ groups of bins in the first level, so size of $U$ is $u= \log^{i+1} n$.
 \vlr{check all the math!}
 
 Let us fix our attention on a bin $b$  in the $i$-th level
 into which some of the elements in group $(i-1, j)$ are distributed after the AKS sort. 
 Consider the pair of pivots $p, q$
 used to determine the contents of bin $b$. This is a successive pair of pivots with label
 pair $(i-1,j)$. Since such a pair splits the elements in group $(i-1,j)$ into $\log n$ bins, 
\elaine{Vijaya, i don't understand why a  pair
of pivots can split the group into log n bins. don't you need log n pivots to do that?} 
these pivots are $r/\log^{i} n$ apart in in sorted sequence of pivots $s[1..r]$.
 Hence the number of elements in array ${\bf I}$ that have ranks between the ranks of these two pivots is
 $k=n/\log^{i+3} n$ (ignoring lower-order additive terms). 
 
 Let $X_b$ be the number of elements in $U$ that have ranks between the ranks of $p$ and $q$.
 These are exactly the elements that are placed in bin $b$.
 $X_b$ is binomially distributed on $k$ elements with success probability 
 $p= k/n = \log^2 n$. Hence, $E[X_b]= u \cdot k/n = \log^2 n$ and using Chernoff bounds,
 $X_b = \log^2 n \pm o(\log^2n)$ with all 
but negligible probability of failure. Thus we have the following lemma.

\elaine{Vijaya: you need the sum 
of Geometric random variables, not the standard Chernoff. also, i thought the last segment
may not satisfy this bound.}
 
 \begin{lemma}\label{lemma-sort-binsize}
 Every bin in {\sc Rec-Sort} has $O(\log^2 n)$ elements placed in it with 
all but negligible (in $n$) probability of failure.
 \end{lemma}
 
 Once we have the $O(\log^2 n)$ bound on the size of any bin, the analysis of {\sc Rec-ORBA} applies
 unchanged to {\sc Rec-Sort} when using AKS for sorting.  Thus, the cost of {\sc Rec-Sort} is
 dominated by the initial call to AKS on $n/\log n$ elements, and it runs with negligible 
 failure probability in optimal $O(n \log n)$ work,
 optimal $O(Q_{\rm sort}(n))$ cache misses 
\elaine{Vijaya: i changed the notation to $Q_{\rm sort}$ to be consistent with later, also
since there are multiple metrics.}
when $M= \Omega (\log^3 n)$, and in $O(\log^2 n)$ span 
 with binary fork-joins.
 
 \vone
 {\bf Using Bitonic Sort.} If we replace AKS with Bitonic Sort in all places in both {\sc Rec-ORBA} and
 {\sc Rec-Sort}, the resulting algorithm is very simple. With a few changes to the algorithm given 
 above, this algorithm will perform $O(n \log n \cdot \log\log n)$ work, which is a $\log\log n$
 factor away from optimal, but the constant factor is extremely small. The parallel time increases from
 $O(\log^2 n)$ to $O(\log^3 n)$, and we attain the optimal $Q_{\rm sort}(n)$ bound 
\elaine{i changed the notation}
for caching if
 $M=\Omega (\log^4 n)$. To chieve this, in the initial sampling step we will sample with probability $1/\log^2n$ in order to ensure that the
 work and caching costs of sorting the sample using bitonic sort remain optimal. In this algorithm we will use bins with $\log^3 n$ elements each, and
 continue to use $\log n$ bins in each group so each small bitonic sort will sort $O(\log^4 n)$ elements.




==> orba-full.tex <==
\section{Summary of Our Sorting Algorithm}\label{sec:orba-sort}

We give an informal overview of our sorting algorithm, deferring
the details to Sections~\ref{sec:warmup} and \ref{sec:rec}.
As mentioned
in the introduction, 
we first 
apply an oblivious random permutation to the input elements,
and then apply any (insecure) {\it comparison-based} sorting algorithm
such as SPMS~\cite{CR17} to the permuted array.
To attain an oblivious random permutation, a key step
is to randomly assign elements to bins of $Z = \omega(\log n)$ 
capacity but without leaking the bin choices --- we call
this primitive oblivious random bin assignment (ORBA). 
For simplicity, we shall assume $Z = \Theta(\log^2 n)$.
%
We now give an overview of our algorithm for ORBA, and then our overall oblivious sorting algorithm.


\subsection{Meta-Algorithm for Random Bin Assignment: {\sc Meta-ORBA} }
\label{sec:summarymetaorba}
Our meta-algorithm for ORBA (henceforth called {\sc Meta-ORBA})
builds on an ORBA algorithm by Asharov et al.~\cite{paracompact} 
and Chan et al.~\cite{cacheoblosort} that 
runs in $O(\log n \cdot \log\log n)$ parallel time on an EREW PRAM
with $O(n \log n)$ work.
In this ORBA algorithm, the $n$ input elements are divided
into $\bins = 2n/Z$ bins and each bin is then padded with $Z/2$ 
filler elements to a capacity of $Z$. 
We assume that 
$\bins$ is a power of 2.
Each real element in the input chooses a random label from the range $[0, \bins-1]$ 
which expresses the desired bin. The elements are then  
routed over a 2-way butterfly network of $\Theta(\log n)$ depth, and in each layer
of the butterfly network there are $\bins$ bins, each of capacity $Z$. 
In every layer $i$ of the network, input bins from the previous layer
are paired up in an appropriate manner, and the real elements  
contained in the two input bins 
are obliviously distributed to two output bins in the next layer, based on the $i$-th bit of
their random labels. For obliviousness, the output bins 
are also padded with filler elements to a capacity of $Z$.


We propose an improvement of the algorithm in~\cite{paracompact} that allows
us to save a $\log \log n$ factor 
in parallel runtime on a PRAM, while retaining work $O(n \log n)$ --- this is our meta-algorithm {\sc Meta-ORBA}.
For this we use a $\Theta(\log n)$-way butterfly network 
rather than $2$-way. Therefore,  
in each layer of the butterfly network, 
groups of $\Theta(\log n)$ input bins\footnote{We assume that 
the branching factor $\Theta(\log n)$ is chosen to be a power of 2.} 
from the previous layer 
are appropriately chosen, 
and the real elements in the $\log n$ input bins are obliviously distributed
to $\Theta(\log n)$ output bins in the next layer, 
based on the next unconsumed $\Theta(\log \log n)$ bits
in their random labels. 
%
Again, all bins are padded with filler elements to a capacity of $Z$
so the adversary cannot tell the bin's actual load.
To perform this $\Theta(\log n)$-way distribution obliviously, 
it suffices to invoke the AKS construction~\cite{aks} 
$O(1)$ number of times (we defer the technical details to Section~\ref{sec:obp}).
Here is a brief analysis of the performance: 

\boi
\item For $O(1)$ invocations of AKS on $\Theta(\log n)$ bins each of size $Z = \Theta(\log^2 n)$:

 Total work is $O(\log^3 n \cdot \log \log n)$ and the parallel time on an EREW PRAM is $O(\log\log n)$.

\item  For computing a single layer, 
there are $\bins /\Theta(\log n)= 2n/\Theta(\log^3 n)$ subproblems: 

 Total work for a single layer is  $O(n\cdot \log \log n)$ and EREW PRAM time remains $O(\log\log n)$.

\item The  $\Theta(\log n)$-way butterfly network has  
$\Theta(\log n/\log\log n)$ layers, 
hence {\sc Meta-ORBA}  performs $O(n\log n)$ total work, and runs in
$O(\log n)$ parallel time on an EREW PRAM.

\eoi

Note that we have improved the parallel runtime by a $\log \log n$ factor
relative to Asharov et al.~\cite{bucketosort} (even when compared
against an improved version of their algorithm that uses 
new primitives such as parallel compaction~\cite{paracompact}).
Although improving the parallel runtime on a PRAM 
is not our final goal, %this same $\log \log n$ improvement 
 the same improvement will translate to an $O(\log \log n)$ factor
saving in span, when we describe our cache-agnostic, binary fork-join implementation 
in Section~\ref{sec:summaryrecorba}.
Without this improvement in the meta-algorithm, 
we will not be able to match 
the best known (insecure) sorting bound in the same computation model.


\subsection{Efficient Cache Agnostic, Binary Fork-Join Implementation}
\label{sec:summaryrecorba}

We now describe {\sc Rec-ORBA}, a recursive cache-agnostic, binary fork-join implementation of our {\sc Meta-ORBA} algorithm.
%
We will assume a tall cache, i.e., $M = \Omega (B^2)$, and we
will also assume $M= \Omega (\log^{1 + \epsilon} n)$ 
for any given arbitrarily small constant $\epsilon >0$. In the following
we will use $\epsilon = 2$ for simplicity, i.e.,  $M = \Omega (\log^3 n)$.

In  {\sc Rec-ORBA},  we 
implement {\sc Meta-ORBA} by recursively solving $\sqrt \bins$ subproblems, 
each with $\sqrt \bins$
bins: in each subproblem, we shall obliviously distribute the  
real elements in the $\sqrt \bins$ 
input bins into $\sqrt \bins$
output bins, using the $(1/2) \log \bins$ most significant bits (MSBs) in the labels.
After this phase, we use a matrix transposition to bring 
the $\sqrt \bins$ 
bins with the same $(1/2) \cdot \log \bins$ MSBs together --- these
$\sqrt \bins$  bins now belong to the same subproblem for the next phase,
where 
we recursively solve each subproblem defined above: for each subproblem, we 
distribute the $\sqrt \bins$  bins into $\sqrt \bins$  output bins
based on the $(1/2) \cdot \log \bins$ least significant bits
in the elements' random labels. 
Since the matrix transposition for $Y$ bins 
each of capacity $Z = \Theta(\log^2 n)$ can be performed
with $O(Y\cdot Z/B)$ cache misses, and $O(\log (Y\cdot Z)) = O(\log n)$
span, we have the %overall caching cost as:
following recurrences that characterize the cost of {\sc Rec-ORBA}
where $Y$ denotes the current number of bins, and $Q(Y)$ 
and $T(Y)$ denote
the cache complexity and span, respectively,  to solve a subproblem 
containing $Y$ bins:
\[
\begin{array}{l}
Q(Y) = 2 \sqrt{Y} \cdot Q(\sqrt{Y}) + O((Y \cdot \log^2 n)/B)\\[5pt]
T(Y) = 2 \cdot T(\sqrt{Y}) + O(\log (Y \cdot \log^2n))
\end{array}
\]

The base conditions are as follows.
Since $M=\Omega (\log^3 n)$ each individual 
$\Theta(\log n)$-way distribution 
instance fits in cache and incurs $O((1/B) \log^3n)$ cache misses. 
Hence we have the base case $Q(Y) = O(Y \log^2 n/B)$ when $Y \log^2 n \leq M$.
For the span, each individual
$\Theta(\log n)$-way distribution instance works on 
$O(\log^3 n)$ elements and has $O( \log^2\log n)$ span under
binary forking, achieved by forking and joining $\log^3 n$ tasks at each level 
of the AKS sorting network. 

Therefore, we have that 
 for $\beta = 2n/Z$: 
$Q(\bins) = O((n/B) \log_M n)$
and $T(\bins) = O(\log n\cdot \log\log n)$. 
Finally, if we want $M = \Omega(\log^{1+\epsilon} n)$ rather
than $M = \Omega(\log^3 n)$, we can simply parametrize 
the bin size to be $\log^{1+\epsilon/2}n$
and let $\gamma = \log^{\epsilon/2}n$.
This gives rise to the following lemma. 


\begin{lemma}\label{orba-recursive}
Algorithm {\sc Rec-ORBA} has cache-agnostic   caching complexity $O((n/B) \log_M n)$ provided the tall cache has
 $M = \Omega (\log^{1+\epsilon} n)$, for any given
positive constant $\epsilon$. The algorithm performs $O(n \log n)$ work and has span $O(\log n \cdot \log\log n)$.
\end{lemma}


\subsection{Full Sorting Algorithm}
\label{sec:summarysort}
From ORBA's output  we obtain $\beta$  bins where
each bin contains real and filler elements. 
To obtain a random permutation of the input array,  it is shown in\cite{cacheoblosort,bucketosort} 
that it suffices to do the following (see Section~\ref{sec:orp} for details):
Assign a $(\log n \cdot \log \log n)$-bit random label to each element, 
and sort the elements 
within each bin based their labels using 
bitonic sort, where all filler elements
are treated as having the label $\infty$ and thus moved to the end of the bin.
Finally, remove the filler elements from all bins, and output the result. 

Let us sort the elements in each bin by their labels with bitonic sort  (with a cost of $O(\log\log n)$ for each comparison due to the large values
 for the labels). Then,
the performance bounds for converting the output of {\sc rec-ORBA} to a random permutation using this method are  dominated by
the bounds for {\sc Rec-ORBA}. So the resulting algorithm generates a random permutation with the same work, span
and cache-oblivious caching bounds as {\sc Rec-ORBA}. (See Section~\ref{sec:schemesort} for details.)

Finally, once the elements have been permuted in random order, 
we can use any insecure comparison-based sorting algorithm 
to sort the permuted array.
We use SPMS sort ~\cite{CR17}, the best cache-agnostic sorting algorithm for the binary fork-join model.
Thus we achieve the bounds in Theorem~\ref{thm:sort},  and we have a data-oblivious sorting algorithm that 
 matches the current best insecure
algorithm in the cache-agnostic binary fork-join model (that is, SPMS itself~\cite{CR17}).  

\begin{theorem}\label{thm:sort}
Sorting $n$ items data-obliviously in the binary fork-join model can be performed in span $O(\log n \cdot \log\log n)$
 with $O(n \log n)$ work and
$O((n/B) \log_M n)$ cache misses cache-agnostically if the tall cache has size $M = \Omega (\log ^{1+\epsilon}n)$, for any given
positive constant $\epsilon>0$.
\end{theorem}



==> scheme.tex <==
%\section{Details of Our Cache-Agnostic, Binary Fork-Join Sorting Algorithm}
%\label{sec:rec}

We describe a new approach to 
implement this meta-algorithm 
%in Section~\ref{sec:warmup}
to achieve cache efficiency in a cache-agnostic model, and
small span.


\subsection{Recursive Random Bin Assignment}
The key step in the meta-algorithm of Section~\ref{sec:warmup} is {\sc Meta-ORBA}.
Therefore, we shall first describe  
a cache-agnostic, binary fork-join implementation of our {\sc Meta-ORBA} algorithm, 
henceforth called {\text{\sc Rec-ORBA}}.

\begin{itemize}[topsep=1pt,itemsep=1pt]
\item 
Upon receiving an input array ${\bf I}$ containing $n := \bins \cdot Z/2$ elements
where $\bins$ is a power of $2$, divide the array ${\bf I}$ into $\bins$
bins each of size $Z/2$. Pad each bin with $Z/2$ filler elements so its size
becomes $Z$.  Let ${\bf I}'$ be the new array 
which is the concatenation of $\bins$ bins each of size $Z$.

\item 
Let $\gamma = \Theta(\log n)$ be a power of $2$.
Call ${\text{\sc Rec-ORBA}}^{\gamma, Z}({\bf I}', 1)$ and output the resulting $\bins$ bins.
The recursive algorithm ${\text{\sc Rec-ORBA}}^{\gamma, Z}$ is defined below. 
\end{itemize}


\begin{mdframed}
\begin{center}
${\text{\sc Rec-ORBA}}^{\gamma, Z}({\bf I}, s)$
\end{center}
\noindent {\bf Input:}
the input contains an array ${\bf I}$
containing $n = \bins \cdot Z$ elements where $\bins$ is assumed to be a power of $2$.
Each element in ${\bf I}$ is either {\it real} or a {\it filler}.
The input array ${\bf I}$ can be viewed as $\bins$ bins each of size $Z$. 
It is promised that each bin has at most $Z/2$ real elements.
Every real element in ${\bf I}$ has a label that determines
which destination bin the element wants to go to.
%For convenience, we write the 
%labels as a separate array ${\sf labels}$, whose length is also $n$.

\vspace{5pt}
\noindent {\bf Algorithm:}

If $\bins \leq \gamma$,  invoke an instance of oblivious bin placement
(Section~\ref{sec:obp})
to assign the input array ${\bf I}$ to a total of $\bins$ bins
each of capacity $Z$. 
Here, each element's destination bin 
is determined by the $s$-th to $(s+\log_2 \bins - 1)$-th bits of its label.
%\elaine{explain earlier in obp what happens if there is overflow.}
%\vlr{Elaine, I do not understand your comment. If it's been addressed, could you remove it?}
Return the resulting list of $\bins$ bins.


Else, proceed with the following recursive algorithm. 
\begin{itemize}[leftmargin=5mm,itemsep=1pt,topsep=1pt]
\item 
Let $\bins_1$ be $\sqrt{\bins}$ rounded up to the nearest power of 2.
Divide the input array ${\bf I}$ into 
$\bins_1$ partitions where each partition 
contains exactly $\bins_2 := \bins/\bins_1$ consecutive bins.
Note that if $\bins$ is a perfect square, $\bins_1 = \bins_2= \sqrt{\bins}$.
Henceforth let ${\bf I}^j$ denote the $j$-th partition where $j \in [\bins_1]$.
\item 
%VLR:
In parallel\footnote{The ``for'' loop is executed in parallel, 
and in the binary fork-join model, a $k$-way parallelism is achieved
by forking $k$ threads in a binary-tree fashion in $\log_2 k$ depth.
In the rest of the paper, we use the same convention when writing pseudo-code
for binary fork-join algorithms; 
%\vlr{Elaine:1) I've added `In parallel'. 2) I'm using fork-join for bitonic sort, so I added this.}
we will use fork and join in the pseudocode for two-way parallelism.}: 
For each $j \in [\bins_1]$, let ${\sf Bin}_{1}^j, \ldots, {\sf Bin}_{\bins_2}^j 
\leftarrow {\text{\sc Rec-ORBA}}^{\gamma, Z}({\bf I}^j, s)$.
\item 
Let ${\sf Bins}$ be a ${\bins_1} \times {\bins_2}$ matrix
where the $j$-th row is the list of bins ${\sf Bin}_{1}^j, \ldots, {\sf Bin}_{\bins_2}^j$.
Note that each element in the matrix is a bin.
Now, perform a matrix transposition: ${\sf TBins} \leftarrow {\sf Bins}^T$.\\
Henceforth, 
let ${\sf TBins}[i]$ denote the $i$-th row of ${\sf TBins}$ consisting of ${\bins_2}$ bins, 
\item 
In parallel: For $i \in [{\bins_2}]$, 
let $\widetilde{\sf Bin}_{1}^i, \ldots, \widetilde{\sf Bin}_{{\bins_1}}^i  
\leftarrow {\text{\sc Rec-ORBA}}^{\gamma, Z}({\sf TBins}[i], s + \log_2 \bins_2 - 1)$
\item 
Return the concatenation 
$\widetilde{\sf Bin}_{1}^1, \ldots, \widetilde{\sf Bin}_{{\bins_1}}^1$, 
$\widetilde{\sf Bin}_{1}^2, \ldots, \widetilde{\sf Bin}_{{\bins_1}}^2$,  
$\ldots$, 
$\ldots$, 
$\widetilde{\sf Bin}_{1}^{{\bins_2}}$, $\ldots$, $\widetilde{\sf Bin}_{{\bins_1}}^{{\bins_2}}$.
\end{itemize}
\end{mdframed}

The intuition is the following --- for convenience, we assume $\beta$ is a perfect square
below (but our formal algorithm description indeed takes care of the case when 
$\beta$ is not a perfect square).
We divide the task of bin assignment
into $\sqrt{\bins}$ sub-problems each of size $\sqrt{\bins}$ (where the size is measured
in terms of bins).
%For each sub-problem, we 
We recursively solve each sub-problem: for each sub-problem, we  
place $\sqrt{\bins} \cdot Z$ elements into  
$\sqrt{\bins}$ bins based on the most significant
$\frac{1}{2} \cdot \log_2 \bins$ bits of their labels.
After this phase, 
since each of the $\sqrt{\bins}$ instances 
outputs $\sqrt{\bins}$ bins, we can view all bins as a $\sqrt{\bins} \times \sqrt{\bins}$ matrix,
where in every column, the elements all share
the same most significant $\frac{1}{2} \cdot \log_2 \bins$ bits of their labels.
We now perform a matrix transposition on this matrix.
Then, each row of the transformed matrix becomes another sub-problem
of size $\sqrt{\bins}$: we recursively solve the sub-problem
defined by each row, and  
assign elements contained in the row to $\sqrt{\bins}$ bins based
on the least significant $\frac{1}{2} \cdot \log_2 \bins$ bits of their labels.


\paragraph{Analysis.}
We now analyze our {\sc Rec-ORBA} algorithm. 
We assume that the cache size $M$
is large enough to hold $\gamma$ bins, that is $M = \Omega(\log^3 n)$.

\begin{itemize}
\item 
{\it Base case:} when the number of bins $\bins \leq \gamma$. 
The base case assigns $\gamma \cdot Z$
elements into $\gamma$ bins based on $\log_2 \gamma$ bits in their labels.
This is achieved by invoking the oblivious bin placement algorithm (see Section~\ref{sec:obp}). 
Since we assume that $M$ is large enough to hold $\gamma$ bins,
we have that 
\[
\text{for } \bins \leq \gamma: 
\begin{array}{l}
W(\bins) = O(\log^3 n \log \log n)\\[5pt]
Q(\bins) = O(\log^3 n /B)\\[5pt]
T(\bins) = O((\log \log n)^2)
\end{array}
\]
where $W(\bins)$ denotes the total work, $Q(\bins)$ denotes the cache complexity,
and $T(\bins)$ denotes the span.

%the base case incurs at most $O(\gamma Z/B) = O(\log^3 n /B)$ cache misses 
%and completes in $O((\gamma Z) \log (\gamma Z)) = O(\log^3 n \log \log n)$
%total work. 

\item 
{\it Recurrence:} when $\bins > \gamma$.
%In this case, we have the following. 
Note that matrix transposition for an $\sqrt{\bins} \times \sqrt{\bins}$ matrix 
where each entry in the matrix is of size $Z = \log^2 n$ 
can be accomplished in $O(\log (\bins Z))$ span, and incurring $O(\bins \cdot Z)$ total work
and $O(\bins Z /B)$ cache misses.
Therefore, in this case, we have the following recurrences:
\[
\text{for } \bins > \gamma: 
\begin{array}{l}
W(\bins) = 2 \sqrt{\bins} \cdot W(\sqrt{\bins}) + O(\bins \log^2 n) \\[5pt]
Q(\bins) = 2 \sqrt{\bins} \cdot Q(\sqrt{\bins}) + O(\bins \log^2 n /B) \\[5pt]
T(\bins) = 2 \cdot T(\sqrt{\bins}) + O(\log (\bins\log^2n))
\end{array}
\]
%Next, we analyze the recurrence. 
\end{itemize}

The above recurrences solve to 
\[
\begin{array}{l}
W(n/Z) = O(n \log n)\\[5pt]
Q(n/Z) = O((n/B) \cdot \log_M n)\\[5pt]
T(n/Z) = O(\log n \cdot \log \log n)\\
\end{array}
\]

Note that the above calculations assume that $\beta$ is a perfect square
in every level of the recursion, but even if not, the 
recurrence would solve to the same asymptotic expressions.

\hide{
\subsection{Random Permutation and Sorting Algorithms}\label{sec:schemesort}

%\elaine{TODO: the previous description was wrong}
%\vlr{Elaine, what does this comment refer to? If it's been addressed please remove your comment and mine.}


\paragraph{{\sc Butterfly-Random-Permute}.}
We use the same algorithm 
as in Section~\ref{sec:orp}
to construct an oblivious random permutation from 
{\sc Rec-ORBA}. We analyze the costs in the binary fork-join model below.
We have $\beta$ parallel sorting problems on $\Theta(\log^2 n)$ elements, where each element has an $O(\log n \cdot \log\log n)$-bit label.
Each sorting problem can be performed  with span $O(\log^4\log  n)$ 
 and work $O(\log^2 n \cdot \log^3 \log n)$ in binary fork-join using bitonic sort by paying a $O(\log\log n)$ factor for the work and span  for each comparison due
to the $O(\log n \cdot \log\log n)$-bit labels. The overall cost for this step across all subproblems
is  $O(n\cdot \log^3 \log n)$ work and the span remains $O(\log^4\log  n)$. Since each bitonic sort subproblem fits in cache, the caching 
cost is simply the scan bound $O(n/B)$.
These bounds are dominated by our bounds for {\sc Rec-ORBA}, 
so this gives an algorithm to generate a random permutation with the same bounds as {\sc Rec-ORBA}.


\paragraph{{\sc Butterfly-Sort}.}
Finally, once the elements have been permuted in random order, 
we can use any insecure comparison-based sorting algorithm 
to sort the permuted array.
We use SPMS sort ~\cite{CR17}, the best cache-agnostic sorting algorithm for the binary fork-join model.
In this way, 
we obtain a data-oblivious
sorting algorithm 
in the cache-agnostic, binary fork-join model,
with optimal cache complexity assuming tall cache and $M= \Omega (\log^{1+\epsilon} n)$,
optimal total work $O(n \log n)$, and 
span $O(\log n \cdot \log\log n)$ which matches the best-known insecure
algorithm in this model (that is, SPMS itself~\cite{CR17}).  

Summarizing the above, we obtain a cache-agnostic and data-oblivious sorting
algorithm with $O(n \log n)$
total work, $O((n/B) \log_M n)$
cache complexity,  and $O(\log n \log \log n)$ span.
This gives our main theorem:

\begin{theorem}[Main theorem]
Assume that the cache size $M \geq \log^3 n$.
Then, there exists a cache-agnostic and data-oblivious sorting algorithm 
that achieves $O(n \log n)$
total work, $O((n/B) \log_M n)$
cache complexity,  and $O(\log n \log \log n)$ span in a binary-fork-join model.
\end{theorem}

}% end hide



==> sort.tex <==

\subsection{Practical and EREW Variants}

So far, our algorithm relies on AKS~\cite{aks} and the SPMS~\cite{CR17} algorithm
as blackbox primitives and thus is not suitable for practical implementation. 
We now describe a practical variant 
that is self-contained and implementable, and gets rid of both AKS and SPMS.
To achieve this, we make two changes --- we outline
the high-level ideas below and defer the details to Appendix~\ref{sec:practical}.

\boi
\item First, we present a simple algorithm to sort a randomly permuted input.
This algorithm {\sc Rec-Sort} uses the same structure as {\sc Rec-Permute} 
but uses a sorted set of pivots to
determine the binning of the elements.  Outside of the need to initially
sort $O(n/\poly\log(n))$ random pivot elements, this algorithm has the same
performance bounds as {\sc Rec-Permute}.

\item Second, we give an improved cache-agnostic, binary fork-join implementation
of bitonic sort. A na\"ive binary fork-join implementation of bitonic sort would incur
$O((n/B)\cdot \log^2 n)$ cache misses and $O(\log^3 n)$ span (achieved by
forking and joining the tasks in each layer in the bitonic network). In our
binary fork-join bitonic sort,  the work remains $O(n \cdot \log^2 n)$ but  the span
reduces to $O( \log^2 n\cdot \log\log n)$ and the caching cost
reduces to $O((n/B) \cdot \log_M n \cdot \log (n/M) )$.
The details are in Appendix~\ref{sec:bitonic}.
\eoi

{\bf Practical Sort.}
By using our improved bitonic sort algorithm in place of AKS networks for small subproblems in
{\sc Butterfly-Permute} and
{\sc Rec-Sort}, we
obtain a simple and practical data-oblivious sorting algorithm that has
optimal cache-agnostic cache complexity if $M = \Omega (\log^{2+\epsilon} n)$
 and incurs only an $O(\log \log n)$ blow-up in work
and an $O(\log n)$ blow-up in span. This algorithm has small constant
factors, with each use of bitonic sort contributing a constant factor of 1/2 to the
bounds for the comparisons made.

\vone
{\bf EREW Butterfly Sort.} For an EREW binary fork-join sorting algorithm, we retain the AKS network in the butterfly computations
in both {\sc Rec-ORBA} and {\sc Rec-Sort}. We continue to use our fork-join bitonic sort for sorting the pivots. Thus the cost
of the overall algorithm is dominated by the cost to sort the $n/\log n$ pivots using bitonic sort,  and we obtain a simple
self-contained EREW binary fork-join sorting algorithm with  the bounds
stated in Theorem~\ref{thm:simple-sort}


Details of our algorithms and their analyses are in Appendix~\ref{sec:practical}, where we establish the following theorem.

\begin{theorem}\label{thm:simple-sort} For $M= \Omega (\log^{2+\epsilon} n)$:\\
(i) The simple practical oblivious sort runs in $O(n \cdot \log n \cdot \log \log n)$ work,  cache-agnostic caching cost $Q_{sort}(n)$,
and $O(\log^2n \cdot \log\log n)$ span.\\
(ii) The EREW Butterfly Sort runs in $O(W_{sort}(n))$ work, cache-agnostic caching cost $O(Q_{sort}(n))$, and 
 $O(\log^2n \cdot \log\log n)$ span.
 \end{theorem}




